AeroTraj: Trajectory Planning for Fast, and Accurate 3D Reconstruction Using a Drone-based LiDAR

This paper presents AeroTraj, a system that enables fast, accurate, and automated reconstruction of 3D models of large buildings using a drone-mounted LiDAR. LiDAR point clouds can be used directly to assemble 3D models if their positions are accurately determined. AeroTraj uses SLAM for this, but must ensure complete and accurate reconstruction while minimizing drone battery usage. Doing this requires balancing competing constraints: drone speed, height, and orientation. AeroTraj exploits building geometry in designing an optimal trajectory that incorporates these constraints. Even with an optimal trajectory, SLAM's position error can drift over time, so AeroTraj tracks drift in-flight by offloading computations to the cloud and invokes a re-calibration procedure to minimize error. AeroTraj can reconstruct large structures with centimeter-level accuracy and with an average end-to-end latency below 250 ms, significantly outperforming the state of the art.

==> 0_metadata.tex <==
% \ifcameraready
% \ifacmartsty
% \begin{CCSXML}
% <ccs2012>
% <concept>
% <concept_id>10003033.10003106.10003112</concept_id>
% <concept_desc>Networks~Cyber-physical networks</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10010520.10010521.10010542.10011714</concept_id>
% <concept_desc>Computer systems organization~Special purpose systems</concept_desc>
% <concept_significance>300</concept_significance>
% </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Networks~Cyber-physical networks}
% \ccsdesc[300]{Computer systems organization~Special purpose systems}
% \fi

% \keywords{Autonomous Cars, ADAS, Collaborative Sensing, Extended Vision}

% \newcommand{\grantack}[1]{
%   \ifthenelse{\equal{#1}{CTA}}{\thanks{Research was sponsored by the Army Research Laboratory and was accomplished under Cooperative Agreement Number W911NF-09-2-0053 (the ARL Network Science CTA). The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}
%     }{}
%   \ifthenelse{\equal{#1}{CRA}}{\thanks{Research reported in this paper was sponsored in part by the Army Research Laboratory under Cooperative Agreement W911NF-17-2-0196. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}}{}
%   \ifthenelse{\equal{#1}{Conix}}{\thanks{This work was supported in part by the CONIX Research Center, one of six centers in JUMP, a Semiconductor Research Corporation (SRC) program sponsored by DARPA.}}{}
%   \ifthenelse{\equal{#1}{NSFAvail}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1705086}}{}
%   \ifthenelse{\equal{#1}{Conix}}{\thanks{This work was supported in part by the CONIX Research Center, one of six centers in JUMP, a Semiconductor Research Corporation (SRC) program sponsored by DARPA.}}{}
%   \ifthenelse{\equal{#1}{CPSSyn}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1330118 and from a grant from General Motors.}}{}        
%   \ifthenelse{\equal{#1}{NeTSLarge}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1413978}}{}         \ifthenelse{\equal{#1}{NeTSSmall}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1423505}}{}
% }

%%% Uncomment one or more of the following
%\grantack{CTA}
%\grantack{CRA}
%\grantack{NSFAvail}
%\grantack{CPSSyn}
%\grantack{NeTSLarge}
%\grantack{NeTSSmall}

\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:



==> back_mot.tex <==
\section{Background \& Motivation}
\label{sec:background_motivation}

% Set up/motivate the problem carefully:
% - Define accuracy and completeness
% - Photogrammetry
% - SLAM
In this section, we will describe the metrics that capture the quality of 3D reconstruction, and results from experiments that motivate \sysname.
% photogrammetry, and SLAM.

\parab{Quantifying 3D model quality. }
Prior work on 3D reconstruction~\cite{reconstructionmetrics} has proposed two metrics, \textit{accuracy} and \textit{completeness}.
Consider a 3D model $M$ and a corresponding ground-truth $M_g$. 
Accuracy describes how \textit{closely} the 3D model $M$ resembles the ground truth $M_g$. 
Accuracy is the root mean square error (RMSE) of the distance from each point in $M$ to the nearest point in $M_g$. 
Completeness describes \textit{what extent} of the ground truth $M_g$ the 3D model $M$ captures.
Completeness is the RMSE of the distance from each point in $M_g$ to the nearest point in $M$. 
% \add{For instance, the right image of \figref{fig:mvs} shows an accurate but incomplete 3D reconstruction obtained using photogrammetry.}

A 10~cm accuracy means that every point on the 3D model $M$ is displaced by 10~cm, on average, from its ground truth position in $M_g$.
A 50~cm completeness means that, on average, for every point on the ground truth $M_g$, the nearest point on the 3D model $M$ is 50~cm away.
If both accuracy and completeness are zero, $M$ perfectly matches $M_g$.
So, for both metrics, \textit{lower is better}. 
These two metrics are roughly analogous to precision (accuracy) and recall (completeness).
% If $M$ captures all points in $M_g$, but the positions of the points are erroneous, then both accuracy and completeness will be non-zero. 
% If $M$ captures only one point in $M_g$, but positions it correctly, its accuracy is perfect, but completeness is poor. 
\add{The right image of \figref{fig:mvs} shows an \textit{accurate but incomplete} 3D reconstruction obtained using photogrammetry.}


% \parab{Photogrammetry.}
% Photogrammetry \textit{infers} 3D models using multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS). MVS algorithms infer the structure (position, and orientation) of the scene from the set of images. Using this structure and stereo correspondence from multiple images, these algorithms estimate the depth of every pixel in each image. A fusion of these 3D points generates a dense 3D reconstruction of the entire scene/object. Though MVS 3D reconstructions are generally accurate, they may contain missing regions or holes~\cite{furukawa15:_multi_view_stereo} which arise if MVS cannot confidently estimate their depths from the set of images.

% \parab{SLAM.}
% SLAM algorithms use 2D/3D sensor data to estimate the pose (position, and orientation) of a robot and build a map of the robot's surroundings, in real-time. LiDAR-based SLAM algorithms continuously align 3D point clouds using scan, and feature matching techniques to precisely estimate the pose (position, and orientation) of the LiDAR/drone. The accuracy of position estimates is directly dependent on SLAM's ability to precisely align 3D point clouds. Alignment, in turn, depends on the nature of the 3D point clouds. For instance, it is relatively easier to align two 3D point clouds for a slow-flying drone because consecutive point clouds are captured in close proximity.  


% \section{Motivation}
% \label{sec:motivation}
% Set up/motivate the problem carefully:
% - Define accuracy and completeness

% - Can use LiDAR, and LiDAR SLAM
%   - Show what happens when we do
%   - SLAM loses tracking
% - Challenge:
%   - Figure out how to minimize tracking loss by trajectory generation
%   - May still have drift; online re-calibrate

% Define Accuracy and Completeness

% In this section, we provide results from experiments that motivate \sysname's approach. 

\begin{figure}[t]
 \centering
  \includegraphics[width=0.5\columnwidth]{figs/fig_incomplete_mvs.pdf}
 \caption{\add{An MVS/photogrammetry-based 3D reconstruction of a building (right image) can be \textit{incomplete} \ie it contains holes and missing regions. The left image shows the ground truth 3D model.}}
 \label{fig:mvs}
\end{figure}

{\small
\begin{table}
  \centering
  % \footnotesize
  % \begin{subtable}{0.45\linewidth}
  \begin{tabular}{{c  c  c  c}} \hline \hline
    \textbf{Building} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} & \textbf{Time (s)} \\ \hline
    % \hline
    Small  & 0.11 & 0.80 & 23084 \\ 
    Large  & 0.16 & 0.75 & 31600 \\ \hline
  \end{tabular}
  \caption{\add{Photogrammetry can be slow, inaccurate and incomplete. The small building is 50m~x50~m~x~20m (length x breadth x height), the large building is 100m~x~50m~x~20m.} 
  % \raj{I might have missed it. Did we mention somewhere that these dimensions represent length~x~breadth~x~height?}
  }
  \label{tab:mvs_motiv}
\end{table}
}

% \parab{Photogrammetry.}
\parab{Drone-based photogrammetry can be slow and inaccurate.} 
% Before
% From a set of images, photogrammetry \textit{infers} 3D models using multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS).
% To do this, it infers the structure (position, and orientation) of a scene.
% Then, it uses the structure along with stereo correspondence from multiple images to estimate the depth of every pixel in each image. 
% A fusion of these 3D points generates a dense 3D reconstruction of the entire scene/object. 
% Though MVS 3D reconstructions are generally accurate, they may be incomplete and contain missing regions or holes~\cite{furukawa15:_multi_view_stereo}.
% This arises if MVS cannot confidently estimate their depths from the set of images.
% Moreover, MVS algorithms are compute-intensive.
% \raj{Should we call "MVS 3D reconstruction" or "MVS-based 3D reconstruction"? If you decide to change, then please change other usages in the paper as well.}
% endBefore
% After
Photogrammetry uses multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS).
MVS infers the scene's 3D structure, and the depth of every pixel in all the images.
Then, it fuses these into a dense 3D reconstruction.
MVS 3D reconstructions are generally accurate, but may contain missing regions or holes (\figref{fig:mvs}) when MVS cannot confidently estimate pixel depths.
Moreover, MVS is also compute-intensive.

% \parab{Drone-based photogrammetry can be slow and inaccurate.} 
\add{
To build a model, an operator flies a drone to collect 2D images.
Then, after landing the drone, the operator uploads them to a cloud service which runs MVS for 3D reconstruction.
}
% Today, to build a 3D model, a drone operator flies a drone to collect 2D images, then lands the drone, and \sout{upload} \addraj{uploads} them to a cloud service which runs MVS to build a 3D model.}
% then upon landing the drone uploads them to a cloud service.
% . Then, the operator uploads these images to a cloud service after the drone lands. 
% The cloud service runs MVS to build a 3D model. 
If the model \textit{contains missing regions} (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. 
It can take multiple iterations to get the desired 3D model. 
% \raj{1st sentence: "to build a 3D model" is repeated twice in the sentence.}


To quantify these shortcomings, we conducted an experiment (methodology described in~\secref{sec:eval}) where we used an open source implementation of MVS (ColMap~\cite{colmap}) to reconstruct 3D models of two buildings. 
For each building, we tried several trajectories, and selected the one that provided the highest quality model. 
% \tabref{tab:mvs_motiv} shows these values, and \figref{fig:mvs} is a visual illustration for that highest quality flight \addraj{model?}. 
% The left image of \figref{fig:mvs} shows the ground truth model, whereas the right image shows the MVS 3D model.
% from the MVS reconstruction. 
MVS accuracy is slightly higher than 10~cm (\tabref{tab:mvs_motiv}); this is desirable. 
Completeness, however, is 75~cm or more.
The right image in \figref{fig:mvs} illustrates incomplete regions in the MVS reconstruction.
\sysname achieves 5 to 9~cm completeness (\secref{sec:eval}), almost an order of magnitude better. 
Finally, MVS requires nearly 7–9 \textit{hours} to reconstruct the model;  \sysname assembles the model in-flight, so the model is ready whilst the drone is in the air.
% immediately after the drone lands.
% \raj{"MVS accuracy is slightly higher than 10~cm; this is desirable. 
% Completeness, however, is 75~cm or more (right image in \figref{fig:mvs} illustrates incomplete regions in the MVS reconstruction); \sysname achieves 5 to 9~cm completeness (\secref{sec:eval}, almost an order of magnitude better)." Simplify this sentence, perhaps too much in brackets is confusing}

\add{
  In theory, photogrammetry could detect, in-flight, when the model is incomplete and adapt the trajectory accordingly. Detecting model incompleteness is challenging without running MVS on the entire set of images~\cite{mostegel2016uav, 7422384}. Thus, in practice, photogrammetry may require iterative data collection. To reduce the number of iterations, companies hire drone pilots or photogrammetrists~\cite{mvslessons, photogrammetryissues} who design trajectories based on their experience and rules of thumb~\cite{colmap, dd_guidelines}. Even so, it is very challenging to ensure complete and high-quality reconstructions without iterations~\cite{mostegel2016uav}. 
}
% As a result, companies often hire experienced drone pilots and photogrammetrists\cite{mvslessons, photogrammetryissues} to design and execute flight trajectories for optimal results.


% In theory, photogrammetry could detect, in-flight, when the model might be incomplete and adapt the trajectory accordingly. This is difficult without running the entire MVS pipeline~\cite{mostegel2016uav, 7422384} on the set of images. 
% To minimize iterations, companies hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} 
% %practitioners 
% have developed rules of thumb for designing trajectories (such as taking highly-overlapping uniformly-illuminated images of texture-rich surfaces)~\cite{colmap, dd_guidelines} and intuitions over time, but realize there is no way to ensure complete and high-quality 3D reconstruction without iteration~\cite{mostegel2016uav}. So, companies hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} who have developed trajectory design intuitions over time.


\parab{Other alternatives for positioning are unsuitable.}
On-board GPS receivers can be used to position point clouds. Unfortunately, GPS errors can range up-to several meters~\cite{gnome}.
% resulting in poor accuracy and completeness of the 3D model. 
The left image of \figref{fig:slam_vs_gps_3d_model} shows a 3D model assembled using a drone flight over a commercial building that uses GPS for positioning; the building's outline is fuzzy, as are the contours of the trees surrounding the building. \tabref{tab:slam_gps_reconstruction} shows that the accuracy and completeness for the GPS reconstructed model are 1.6~m and 0.53~m, respectively, both of which are undesirable. The right image of \figref{fig:slam_vs_gps_3d_model} shows a 3D reconstruction using techniques proposed in this paper, which does not use GPS. 
% (All reconstructions in \figref{fig:slam_vs_gps_3d_model} use real data captured from a drone-mounted LiDAR~\secref{sec:eval}).

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/fig_slam_vs_gps_3d_model.pdf}
    \caption{\add{Three models of a large complex on our campus: GPS (left), SLAM (middle), and \sysname (right). All models use the same height ramp function to color-code the z-axis, with blue representing the lowest points and orange representing the highest. The \sysname model has distinct features and trees, with clear and crisp coloring, indicating a good reconstruction. In contrast, the GPS and SLAM models have diffused colors and lack visible features, suggesting poor and noisy reconstruction.}}
    \label{fig:slam_vs_gps_3d_model}
\end{figure}

{\small
\begin{table}
  \begin{tabular}{{c c c c}} \hline \hline
    \textbf{Approach} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} & \add{\textbf{Flight time (s)}} \\ \hline
    % \hline
    GPS  & 1.60 & 0.53 & \add{944} \\ 
    SLAM  & 2.30 & 1.30 & \add{944} \\ 
    \sysname & 0.13 & 0.09 & \add{750} \\ \hline
  \end{tabular}
  \caption{Relative to \sysname, alternative reconstruction approaches for drone-based LiDAR reconstruction give poor quality 3D models.}
  \label{tab:slam_gps_reconstruction}
\end{table}
}

High-precision GNSS/RTK receivers can provide more accurate positioning but require additional infrastructure, are costly, and can perform poorly (tens of meters of error~\cite{Carloc}) in urban environments. 
Prior work~\cite{uav_lidar_1,uav_lidar_2} has used such receivers in \textit{remote sensing}, for \textit{offline} reconstruction, using specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors.
% (but for \textit{offline} model reconstruction). 
In contrast, we consider solutions that employ off-the-shelf technologies: drones, and commodity GPS and LiDAR for online reconstruction.

\parab{SLAM-based positioning on a drone is challenging.}
LiDAR-based SLAM algorithms continuously align 3D point clouds using scan~\cite{Cartographer}, and feature matching~\cite{zhang2014loam,liosam} techniques to precisely estimate the pose (position, and orientation) of the LiDAR/drone. The accuracy of position estimates is dependent on SLAM's ability to precisely align 3D point clouds. Alignment, in turn, depends on the nature of the 3D point clouds. For instance, it is relatively easier to align two 3D point clouds for a slow-flying drone because consecutive point clouds are captured in close proximity. 
\raj{"because consecutive point clouds are captured in close proximity" -> "because consecutive point clouds have good overlap"}
% Precise positioning with SLAM is challenging on a drone as compared to autonomous vehicles
% In contrast to autonomous vehicles, drone-based SLAM is challenging due to the significantly sparser 3D point clouds generated by the drone LiDAR as compared to a vehicle-mounted LIDAR.
% Sparsity makes aligning point clouds challenging, resulting in imprecise positioning.
% Although SLAM is used in autonomous driving (among other applications) for precise positioning, it is challenging to use it out-of-the-box on a drone. 
% When mounted on a drone, a LiDAR generates significantly sparser 3D point clouds as compared to a vehicle.
% Sparsity makes it difficult for the SLAM algorithm to align the point clouds, resulting in imprecise positioning.
\add{To understand the importance of LiDAR alignment, consider \figref{fig:slam_challenge}. The scan plane of a vehicle LiDAR (\figref{fig:slam_challenge} (A)) is parallel to the ground; the central laser beams run parallel to the ground. This way, the LiDAR receives numerous returns (solid orange lines) from objects in the surrounding \eg the road, traffic signs, and buildings \etc
  This results in dense point clouds, better alignment and hence accurate SLAM positioning.
  With a parallel mount on a drone at height $h$ (\figref{fig:slam_challenge} (B)), the LiDAR exhibits significantly fewer returns, if any.
When the scan plane is perpendicular to the ground (\figref{fig:slam_challenge} (C)), the LiDAR receives relatively more returns.
Even then, these returns are only 9\% of the returns from a vehicle mounted LiDAR.
With sparse returns, SLAM cannot precisely align consecutive point clouds and hence results in imprecise and inaccurate positioning.
This can be overcome with careful \textit{trajectory design} that can ensure significant overlap between point clouds so SLAM can position accurately.
% As such, positioning accuracy in SLAM is critically dependent on the drone's \textit{flight trajectory}.
}

\raj{In the paper, I feel that too much text are in brackets which disturbs the flow during reading.}

\begin{figure}[t]
\centering
\begin{minipage}{0.65\linewidth}
 \centering\includegraphics[width=0.80\textwidth]{figs/fig_slam_challenge.pdf}
 \caption{LiDAR returns when mounted on a vehicle (A) and a drone platform (B and C). The solid lines indicate the lasers have hit an object, whereas the dotted lines that those laser beams did not hit any object.}
 \label{fig:slam_challenge}
\end{minipage}
\hfill
\begin{minipage}{0.3\linewidth}
 \includegraphics{figs/rectflight.png}
 \caption{Rectilinear trajectory for SLAM-based reconstruction.}
 \label{fig:rectflight}
\end{minipage}
% \caption{}
\end{figure}

%before
% \figref{fig:slam_vs_gps_3d_model} (middle) shows reconstruction using SLAM from a rectilinear flight (\figref{fig:rectflight}) that ensures building coverage. For this flight, the accuracy, and completeness are 2.3~m and 1.3~m respectively (\tabref{tab:slam_gps_reconstruction}, lower values of accuracy and completeness are better), orders of magnitude higher than \sysname-based reconstruction. 
% This reconstruction is visually worse than \sysname-based reconstruction (\figref{fig:slam_vs_gps_3d_model} (right)), because the underlying SLAM algorithm is unable to \textit{track} LiDAR frames (\ie it is unable to match points in successive point clouds). 
% \sysname, which layers trajectory generation and drift re-calibration on top of SLAM, is significantly more accurate and complete. 
% For SLAM-based reconstructions, we used the Google Cartographer~\cite{Cartographer} LiDAR SLAM implementation which uses scan matching.
%endbefore

To quantify this, we used a rectilinear flight (\figref{fig:rectflight}) to build a 3D model of a large building using the Google Cartographer LiDAR SLAM~\cite{Cartographer} implementation.
The resulting 3D model has 2.3~m accuracy, 1.3~m completeness (\tabref{tab:slam_gps_reconstruction}), and is visually worse (\figref{fig:slam_vs_gps_3d_model} (right)) than \sysname-based reconstruction.
SLAM cannot align successive point clouds and hence results in imprecise pose estimates.
\sysname, which layers trajectory generation and drift re-calibration on top of SLAM, is significantly more accurate and complete.
% F
\raj{"is significantly more accurate and complete." -> "creates significantly more accurate and complete 3D models."}

\parab{Limited compute on drones.}
For \sysname to detect SLAM drift (\secref{sec:intro}) in-flight, it must run SLAM as the drone flies. 
% However, existing SLAM algorithms \textit{cannot run at full frame rate} on mobile computing platforms mounted on drones. 
A DJI M600Pro (which we use in this paper) hexacopter has a maximum payload weight of 5~kg. 
% It carries an A3Pro flight controller that contains three IMUs and three GNSS receivers. 
On this, we mounted an LTE radio, an Ouster OS1-64 LiDAR and a Jetson TX2 board.
This compute capability is far from sufficient to run LiDAR SLAM at full-frame rate\footnote{With a 64-beam LiDAR, SLAM processes up to 480 Mbps of 3D data}. 

On the TX2, we ran two popular, representative LiDAR-SLAM algorithms, Cartographer~\cite{Cartographer} and LOAM~\cite{zhang2014loam}.
In this experiment, both SLAM implementations use \sysname's optimized 3D flight trajectories. In \tabref{tab:lidar_slam_compute} we show accuracy, completeness and performance results for two of the LiDAR SLAM algorithms. 
Cartographer, a scan matching algorithm, can only process 2 frames per second (LiDARs generate 10–20 frames per second) and LOAM, a feature-matching algorithm, can process 5 frames per second. Though faster, LOAM reconstructions are worse than Cartographer.

\begin{table}[t]
  % \footnotesize
  \centering
  \begin{tabular}{c  c  c} \hline \hline 
    \textbf{Metric} & \textbf{Cartographer~\cite{Cartographer}} & \textbf{LOAM~\cite{zhang2014loam}} \\ \hline
    % \hline
    Frame Rate (fps) & 2 & 5 \\ 
    Accuracy (m) & 0.21 & 5.75 \\ 
    Completeness (m) & 0.09 & 2.74 \\ \hline
  \end{tabular}
  \caption{LiDAR SLAM on Jetson TX2. For both accuracy and completeness, lower is better.}
  \label{tab:lidar_slam_compute}
\end{table}

We make two observations from \tabref{tab:lidar_slam_compute}.
First, Cartographer is a more accurate than LOAM for drone-mounted LiDAR SLAM. For this reason, \sysname uses Cartographer.
Second, neither \addraj{of the two SLAM implementations} can run at full frame-rate on the drone. In particular, Cartographer runs only at 2~fps, but we need to process SLAM at full-frame rate to be able to detect drift in-flight, so \sysname offloads SLAM to the cloud.
\raj{"Cartographer is more accurate than LOAM" or "Cartographer is a more accurate SLAM implementation than LOAM"}
These experimental results motivate the design of \sysname, which we now describe.



==> background.tex <==
\section{Background}
\label{sec:background}
% Set up/motivate the problem carefully:
% - Define accuracy and completeness
% - Photogrammetry
% - SLAM
In this section, we will describe the metrics that capture the quality of 3D reconstruction, photogrammetry, and SLAM.

\parab{Quantifying 3D model quality. }
Prior work on 3D reconstruction~\cite{reconstructionmetrics} has proposed two metrics, \textit{accuracy} and \textit{completeness}.
Consider a 3D model $M$ and a corresponding ground-truth $M_g$. 
Accuracy describes how \textit{closely} the 3D model $M$ resembles the ground truth $M_g$. 
Accuracy is the root mean-square error (RMSE) of the distance from each point in $M$ to the nearest point in $M_g$. 
Completeness describes \textit{what extent} of the ground truth $M_g$ the 3D model $M$ captures.
Completeness is the RMSE of the distance from each point in $M_g$ to the nearest point in $M$. 
\add{For instance, the right image of \figref{fig:mvs} shows an accurate but incomplete 3D reconstruction obtained using photogrammetry.}

To put these numbers in context, a 10~cm accuracy means that every point on 3D model $M$ is displaced by 10~cm, on average, from its ground truth position in $M_g$.
% A high accuracy value means the 3D model $M$ does not resemble the ground truth $M_g$.
A 50~cm completeness means that, on average, for every point on the ground truth $M_g$, the nearest point on the 3D model $M$ is 50~cm away.
% A high completeness value means the 3D model $M$ is an incomplete representation of the ground truth $M_g$.
If both accuracy and completeness are zero, $M$ perfectly matches $M_g$.
So, for both metrics, \textit{lower is better}. 
If $M$ captures all points in $M_g$, but the positions of the points are erroneous, then both accuracy and completeness will be non-zero. 
If $M$ captures only one point in $M_g$, but positions it correctly, its accuracy is perfect, but completeness is poor. 
These two metrics are roughly analogous to precision (accuracy) and recall (completeness).
% \fawad{Consider adding a figure to show how these metrics work. Maybe with MVS}

% \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{figs/fig_incomplete_mvs.pdf}
%  \caption{MVS reconstruction (right image) of a large building (left image shows ground truth 3D model).}
%  \label{fig:mvs}
% \end{figure}


% \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{figs/fig_slam_challenge.pdf}
%  \caption{LiDAR returns when mounted on a vehicle and a drone platform}
%  \label{fig:slam_challenge}
% \end{figure}


% \begin{table}[t]
%   \centering
%   \footnotesize
%   \begin{tabular}{{|c | c | c | c|}} \hline
%     \textbf{Building} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} & \textbf{Time (s)} \\ \hline
%     % \hline
%     Small  & 0.11 & 0.80 & 23084 \\ \hline
%     Large  & 0.16 & 0.75 & 31600 \\ \hline
%   \end{tabular}
%   \caption{Photogrammetry can be slow and inaccurate. The small building is 50~m~x~50~m~x~20~m, the large is 100~m~x~50~m~x~20~m.}
%   \label{tab:mvs_motiv}
% \end{table}

\parab{Photogrammetry.}
Photogrammetry \textit{infers} 3D models using multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS). MVS algorithms infer the structure (position, and orientation) of the scene from the set of images. Using this structure and stereo correspondence from multiple images, these algorithms estimate the depth of every pixel in each image. A fusion of these 3D points generates a dense 3D reconstruction of the entire scene/object. Though MVS 3D reconstructions are generally accurate, they may contain missing regions or holes~\cite{furukawa15:_multi_view_stereo} which arise if MVS cannot confidently estimate their depths from the set of images.

\parab{SLAM.}
SLAM algorithms use 2D/3D sensor data to estimate the pose (position, and orientation) of a robot and build a map of the robot's surroundings, in real-time. LiDAR-based SLAM algorithms continuously align 3D point clouds using scan, and feature matching techniques to precisely estimate the pose (position, and orientation) of the LiDAR/drone. The accuracy of position estimates is directly dependent on SLAM's ability to precisely align 3D point clouds. Alignment, in turn, depends on the nature of the 3D point clouds. For instance, it is relatively easier to align two 3D point clouds for a slow-flying drone because consecutive point clouds are captured in close proximity.  

% % Today, to build a 3D model, a drone operator flies a drone in a given trajectory to collect 2D images. Then, the operator uploads these images to a cloud service after the drone lands. The cloud service runs an MVS algorithm to build a 3D model. If the model contains missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive.

% % To quantify these shortcomings, we conducted an experiment (methodology described in~\secref{sec:eval}) in which we used an open source implementation of MVS (ColMap~\cite{colmap}) to reconstruct a 3D model of two buildings. For each building, we tried several trajectories, and selected the one that provided the highest quality model. \tabref{tab:mvs_motiv} shows these values, and \figref{fig:mvs} is a visual illustration for that highest quality flight. 
% % % \figref{fig:mvs} is a visual illustration of highest quality flight MVS reconstruction. 
% % The left image shows the ground truth model whereas the right image shows the 3D model from the MVS reconstruction. Accuracy is slightly higher than 10~cm; this is desirable. Completeness, however, even for the best flight is 75~cm or more (right image in \figref{fig:mvs} illustrates many regions in the MVS reconstruction are incomplete); \sysname achieves 5 to 9~cm completeness (\secref{sec:eval}, almost an order of magnitude better). Finally, MVS requires nearly 7-9 \textit{hours} to reconstruct the model;  \sysname assembles the model in-flight, so the model is ready immediately after the drone lands.




% In theory, photogrammetry could detect, in-flight, when the model might be incomplete and adapt the trajectory accordingly. This has proven to be hard to do without running the entire MVS pipeline~\cite{mostegel2016uav, 7422384} on the set of images. To minimize iterations, practitioners have developed rules of thumb for designing trajectories (such as taking highly-overlapping uniformly-illuminated images of texture-rich surfaces)~\cite{colmap, dd_guidelines}, but realize there is no way to ensure complete and high-quality 3D reconstruction without iteration~\cite{mostegel2016uav}. So, companies hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} who have developed trajectory design intuitions over time.



% \parab{Other alternatives for positioning are unsuitable.}
% Because drones can carry GPS receivers, GPS can be used to position point clouds. Unfortunately, GPS errors can range up-to several meters~\cite{gnome}, resulting in poor accuracy and completeness of the 3D model. The left image of \figref{fig:slam_vs_gps_3d_model} shows a 3D model of a building assembled using a drone flight over a commercial building that uses GPS for positioning; the building's outline is fuzzy, as are the contours of the trees surrounding the building. \tabref{tab:slam_gps_reconstruction} shows that the accuracy and completeness for the GPS reconstructed model are 1.6~m and 0.53~m respectively, both of which are undesirable. The right image shows a 3D reconstruction using techniques proposed in this paper, which does not use GPS. (All reconstructions in \figref{fig:slam_vs_gps_3d_model} use real data captured from a drone-mounted LiDAR~\secref{sec:eval}).

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/fig_slam_vs_gps_3d_model.pdf}
%     \caption{GPS (left), SLAM (middle), and \sysname (right) derived models of a large complex on our campus. All models are color-coded with the same height ramp function.}
%     \label{fig:slam_vs_gps_3d_model}
% \end{figure}

% \begin{table}[t]
%   \centering
%   \footnotesize
%   \begin{tabular}{{|c|c|c|}} \hline
%     \textbf{Approach} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} \\ \hline
%     % \hline
%     GPS  & 1.60 & 0.53 \\ \hline
%     SLAM  & 2.30 & 1.30 \\ \hline
%     \sysname & 0.13 & 0.09 \\ \hline
%   \end{tabular}
%   \caption{Relative to \sysname, alternative reconstruction approaches for drone-based LiDAR reconstruction give poor quality 3D models.}
%   \label{tab:slam_gps_reconstruction}
% \end{table}

% \ramesh{Do we have acc/compl for GPS?}
% \fawad{Yes, but we have it for the real-world building not the Airsim ones. I added the numbers in the paragraph above.}

% High-precision GNSS/RTK receivers can provide more accurate positioning but require additional infrastructure, are costly, and can perform poorly (tens of meters error~\cite{Carloc}) in urban environments due to non line-of-sight signals that degrade accuracy. Prior work~\cite{uav_lidar_1,uav_lidar_2} has used expensive GPS receivers in the context of \textit{remote sensing}, using specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors (but for \textit{offline} model reconstruction). In contrast, in this paper we consider solutions that employ off-the-shelf technologies: drones, and commodity GPS and LiDAR for online reconstruction.

% \parab{SLAM-based positioning on a drone is challenging.}
% Although SLAM is used in autonomous driving (among other applications) for precise positioning, it is challenging to use it out-of-the-box on a drone. 
% When mounted on a drone, a LiDAR generates significantly sparser 3D point clouds as compared to a vehicle.
% Sparsity makes it difficult for the SLAM algorithm to align the point clouds, resulting in imprecise positioning.
% Consider an 8-beam LiDAR as shown in \figref{fig:slam_challenges}.
% These laser beams are radially placed on a rotating platform in a mechanical closure.
% Each laser beam shoots laser pulses in 360\degree.
% Because the lasers are radially placed, the beams diverge as their distance from the LiDAR increases.
% % These laser beams are radially placed in the mechanical enclosure of the LiDAR.
% Thereby, the LiDAR receives more returns from the same object when placed closeby as opposed to when it placed far away.
% % Objects closeby to the LiDAR generate more returns because the LiDAR beams have not yet dispersed.
% % Objects that are far away generate fewer returns because LiDAR beams have dispersed.

% On a vehicle, the LiDAR is placed such that scan plane of the LiDAR is parallel to the ground.
% What this means is: the central laser beams of the LiDAR are parallel to the ground.
% In this positioning, the vehicle-mounted LiDAR gets returns from numerous objects \eg the road, traffic signs, buildings, other vehicles \etc
% % because the vehicle has objects closeby, the LiDAR generates a lot of returns.
% On a drone, however, if the LiDAR is placed in the same orientation, it will have hardly any returns as depicted in \figref{fig:slam_challenges} because the drone is in-flight.
% A different way to orient the LiDAR is to position it such that the scan plane of the LiDAR is perpendicular to the ground.
% In this orientation, the LiDAR receives relatively more returns.
% However, these returns are only 1/10th of the returns when the LiDAR is mounted on a vehicle.
% As such, positioning accuracy in SLAM critically depends on the drone's \textit{flight trajectory}.
% As such, with sparse returns, SLAM cannot precisely align consecutive point clouds and hence results in imprecise and inaccurate positioning.

% % \figref{fig:slam_challenges} illustrates the positioning of a LiDAR on a vehicle and a drone. On a vehicle, as the 

% \parab{SLAM-based positioning can be inaccurate.}
% Even with SLAM, reconstruction quality is critically dependent on the design of the drone \textit{trajectory}. \figref{fig:slam_vs_gps_3d_model} (middle) shows reconstruction using SLAM from a rectilinear flight (\figref{fig:rectflight}) that ensures building coverage. For this flight, the accuracy and completeness are 2.3~m and 1.3~m respectively (\tabref{tab:slam_gps_reconstruction}, lower values of accuracy and completeness are better), orders to magnitude higher than \sysname-based reconstruction. This reconstruction is visually worse than \sysname-based reconstruction (\figref{fig:slam_vs_gps_3d_model} (right)), because the underlying SLAM algorithm is unable to \textit{track} LiDAR frames (\ie it is unable to match points in successive point clouds). \sysname, which layers trajectory generation and drift re-calibration on top of SLAM is significantly more accurate and complete. For SLAM-based reconstructions, we used the Google Cartographer~\cite{Cartographer} LiDAR SLAM implementation.

% \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.35\columnwidth]{figs/rectflight.png}
%  \caption{Rectilinear trajectory for SLAM-based reconstruction.}
%  \label{fig:rectflight}
% \end{figure}

% % To quantify the quality of SLAM-based reconstruction, we measured accuracy and completeness for the two buildings discussed above. These experiments (and all others in this paper) use Google's Cartographer~\cite{Cartographer}, a recent implementation of LiDAR SLAM. As \tabref{tab:slam_motiv} shows, SLAM-based reconstruction has worse accuracy than MVS, but better completeness. \sysname, which layers trajectory generation and drift re-calibration on top of SLAM is significantly more accurate and complete (\secref{sec:eval}).

% % \fawad{These numbers are very low (they need to be higher). They represent \sysname without re-calibration. For GPS and unoptimized SLAM, maybe we can just use numbers from the real-world trace instead?}
% % \begin{table}[h]
% %   \small
% %   \centering
% %   \begin{tabular}{{|l|c|c|c|}} \hline
% %     Building & Accuracy (m) & Completeness (m)  \\ \hline\hline
% %     Small  & 0.25 & 0.14 \\ \hline
% %     Large  & 0.21 & 0.24 \\ \hline
% %   \end{tabular}
% %   \caption{SLAM-based reconstruction can be inaccurate. The dimensions of the buildings are as in \tabref{tab:mvs_motiv}.}
% %   \label{tab:slam_motiv}
% % \end{table}


% % \noindent$\blacktriangleright$
% \parab{Limited compute on drones.}
% For \sysname to detect SLAM drift (\secref{sec:intro}) in-flight, it must run SLAM as the drone flies. However, existing SLAM algorithms \textit{cannot run at full frame rate} on mobile computing platforms mounted on drones. A DJI M600Pro (which we use in this paper) hexacopter has a maximum payload weight of 5~kg. It carries an A3Pro flight controller that contains three IMUs and three GNSS receivers. We have also mounted an LTE radio and an Ouster OS1-64 LiDAR, as well as a Jetson TX2 board. This compute capability is far from sufficient to run LiDAR SLAM\footnote{With a 64-beam LiDAR, SLAM processes upto 480 Mbps of 3D data}. 

% On the TX2, we ran two popular, representative LiDAR-SLAM algorithms, Cartographer~\cite{Cartographer} and LOAM~\cite{zhang2014loam}.
% In this experiment, both SLAM implementations use \sysname's optimized 3D flight trajectories. In \tabref{tab:lidar_slam_compute} we show accuracy, completeness and performance results for two the LiDAR SLAM algorithms. 
% Cartographer, a scan matching algorithm, can only process 2 frames per second (LiDARs generate 10-20 frames per second) and LOAM, a feature-matching algorithm, can process 5 frames per second. Though faster, LOAM reconstructions are worse than Cartographer.

% \begin{table}[t]
%   \footnotesize
%   \centering
%   \begin{tabular}{|c | c | c|} \hline 
%     \textbf{Metric} & \textbf{Cartographer~\cite{Cartographer}} & \textbf{LOAM~\cite{zhang2014loam}} \\ \hline
%     % \hline
%     Frame Rate (fps) & 2 & 5 \\ \hline
%     Accuracy (m) & 0.21 & 5.75 \\ \hline
%     Completeness (m) & 0.09 & 2.74 \\ \hline
%   \end{tabular}
%   \caption{LiDAR SLAM on Jetson TX2. For both accuracy and completeness, lower is better.}
%   \label{tab:lidar_slam_compute}
% \end{table}

% We make two observations from \tabref{tab:lidar_slam_compute}.
% First, Cartographer is a more accurate SLAM algorithm than LOAM for drone-mounted LIDAR. For this reason, \sysname uses Cartographer.
% Second, neither SLAM implementation can run at full frame-rate on the drone. In particular, Cartographer runs only at 2~fps, but we need to process SLAM at full-frame rate to be able to detect drift in-flight, so \sysname offloads SLAM to the cloud.

% In the future, mobile compute capabilities will improve. However, at the same time, LiDAR technology continues to evolve and 128 beam LIDARs are already available, and these will require significantly more compute. So it is unclear if, or when, accurate LiDAR SLAM can run entirely on the drone. Even if that becomes feasible, \sysname's trajectory optimization and re-calibration algorithms will be relevant for accurate 3D modeling.

% \parab{Mobile device LiDAR-based reconstruction is infeasible. }
% \sysname could have used LiDARs now available on mobile devices (\eg iPhones) to perform 3D reconstruction. However, LiDARs on mobile devices work well only in indoor environments because: a) the mobile device LiDAR has a limited sensing range of about 3~m~\cite{iphone_depth}, and b) has high depth estimation errors beyond this range \eg up to 30~cm at 4~m~\cite{iphone_depth2}.  In outdoor spaces, these approaches can have tracking errors in meters~\cite{iphone_tracking} which leads to undesirable results.

% Even with perfect tracking, to capture a large physical structure (\eg a building) a drone with a mobile device based LiDAR will have to fly longer because of its sensing limited range. This can easily exhaust the drone's battery. Our calculations show that, for such an approach, reconstructing a large building (\eg a 100m~x~50m~x~20m building, \secref{sec:eval}) can take several hours of the drone flight time. Drones that can carry payloads have less than 30 minutes~\cite{drone_payloads} of flight time in a single battery cycle (the DJI M600Pro, which we use in this paper, has a flight time of 25 minutes).

% % \ramesh{For the last sentence, it might be better to also include flight duration for lighter drones on which smartphones might be mounted?}

% % Cartographer cannot run at full frame-rate on the droneSecond, LiDAR SLAM algorithms cannot run at full frame-rate on the drone compute.

% These experimental results motivate the design of \sysname, which we now describe.


% % Two metrics define the quality of a 3D model. 
% % \textit{Accuracy} quantifies how closely a 3D model replicates a physical object (see \secref{s:slam-phase} for a more precise definition).
% % It is the average Euclidean distance between the positions of every point in the 3D model to the corresponding point on the surface of the physical object (see \secref{s:slam-phase} for a more precise definition).
% % A 3D model with an accuracy of 0~m perfectly replicates a physical object.
% % \textit{Completeness} quantifies the degree to which a model captures the entire physical object (see \secref{s:slam-phase} for a more precise definition).
% % It is the inverse of accuracy \ie it is the average Euclidean distance between the position of every point on the surface of the physical object to the corresponding point on the 3D model.
% % A 3D model with 0~m completeness is completely perfectly a physical object.

% % Photogrammetry
% % - Show MVS doesn't work, and why
% %   - Don't know which part is not captured well (do we have some examples)
% % \parab{Multi-View Stereo (MVS). }
% % % Photogrammetry uses multi-view stereo algorithms to infer a 3D model from drone captured 2D images.
% % % MVS takes too long and there is no feedback signal into how the reconstruction is going.
% % % Mostly using photogrammetry.
% % Most existing work (\secref{sec:related}) use \textit{photogrammetry} to infer a 3D model from 2D images.
% % Photogrammetry uses multi-view stereo~\cite{furukawa15:_multi_view_stereo}, which takes as input a sequence of 2D camera images (and the positions associated with these images), captured either using drone-mounted cameras~\cite{7139681, 7989530, 8124461, 8628990} or by humans using ordinary mobile devices~\cite{company_hover}. 
% % % Photogrammetry \textit{infers} 3D models using multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS). 
% % MVS algorithms infer the structure (position, and orientation) of the scene from the set of images (called structure from motion or SfM). 
% % Using this structure and stereo correspondence from multiple images, these algorithms estimate the depth of every pixel in each image. 
% % A fusion of these 3D points generates a dense 3D reconstruction of the entire scene/object.

% % \parab{No feedback signal in MVS. }
% % Though MVS 3D reconstructions are generally accurate, they may contain missing regions or holes~\cite{furukawa15:_multi_view_stereo} which arise if MVS cannot confidently estimate their depths from the set of images.

% % Collect good images or have an expert do it and hope for the best.
% %Besides some generic rules of thumb for collecting images (\eg texture-rich, uniform illuminated images with high overlap taken from diverse viewpoints)~\cite{colmap, dd_guidelines}, there is no way to ensure complete and high-quality 3D reconstruction~\cite{mostegel2016uav}. Companies, besides issuing these guidelines,  hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} for data collection who have developed intuition over time for better trajectory design.

% % It feels important to talk about this work but it might also raise questions about our contributions from the very start. I am not sure if we should keep it or remove it (it is already present in the related work section)
% % There is work~\cite{cvpr} that trains a model to predict the likelihood of a good/complete 3D model from a set of images. However, this model is specific to a given dataset and a given MVS algorithm. For a different scene or MVS algorithm, the model will need to be trained again with a new set of labeled data.

% % MVS takes too long and there is no feedback signal into how the reconstruction is going.
% % Today, to build a 3D model, a drone operator flies a drone in a given trajectory to collect 2D images. Then, the operator uploads these images to a cloud service after the drone lands. The cloud service runs an MVS algorithm to build a 3D model. If the model contains missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive. On a relatively powerful GPU workstation, reconstructing a building takes upto 8~hours (\secref{sec:eval}). As such, multiple iterations can result in a turnaround time of several days.

% % \parae{The need for trajectory adaptation.}
% % In theory, photogrammetry can avoid this iterative approach if it could detect, in-flight, when the model might be incomplete and adapt the trajectory accordingly. This has proven to be hard to do without running the entire MVS pipeline~\cite{mostegel2016uav, 7422384} on the set of images. To minimize  iterations, practitioners have developed rules of thumb for designing trajectories (such as taking highly-overlapping uniformly-illuminated images of texture-rich surfaces from diverse viewpoints)~\cite{colmap, dd_guidelines}, but realize there is no way to ensure complete and high-quality 3D reconstruction without iteration~\cite{mostegel2016uav}. For this reason, companies hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} who have developed trajectory design intuitions over time.

% % Today, to build a 3D model, a drone operator flies a drone in a given trajectory to collect 2D images. Then, the operator uploads these images to a cloud service after the drone lands. The cloud service runs an MVS (multi-view stereo) algorithm to build a 3D model. If the model contains missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive. On a relatively powerful GPU workstation, reconstructing a building takes upto 8~hours (\secref{sec:eval}). As such, multiple iterations can result in a turnaround time of several days.



==> contributions.tex <==
\subsection{Challenges and Contributions}
\label{sec:contributions}

% \parab{
%   Challenges.}
\parab{Challenges.}
Using SLAM on drone-mounted LiDAR is challenging for the following reasons (\tabref{tab:challenges}).

% \paraspace\noindent$\blacktriangleright$
\parae{Trajectory design.}
Reconstruction quality is critically dependent on the design of the drone \textit{trajectory}. \figref{fig:slam_vs_gps_3d_model} (middle) shows reconstruction using SLAM from a poorly planned drone flight. This reconstruction is visually worse than GPS-based reconstruction (\figref{fig:slam_vs_gps_3d_model} (left)), because the underlying SLAM algorithm is \textit{unable to track} LiDAR frames (\ie it is unable to match points in successive point clouds).

% \noindent$\blacktriangleright$
\parae{Drift.}
SLAM algorithms \textit{accumulate drift}~\cite{slam_part1,slam_part2}, so position estimates can degrade on longer flights.

\begin{table}[t]
  \footnotesize
  \centering
  \begin{tabular}{|c|c|c|} \hline 
    & \textit{\textbf{Cartographer~\cite{Cartographer}}} & \textit{\textbf{LOAM~\cite{zhang2014loam}}} \\ \hline \hline
    Frame Rate (fps) & 2 & 5 \\ \hline
    Accuracy (m) & 0.21 & 0.09 \\ \hline
    Completeness (m) & 5.75 & 2.74 \\ \hline
  \end{tabular}
  \caption{LiDAR SLAM on mobile compute platform (Jetson TX2)}
  \label{tab:lidar_slam_compute}
\end{table}

% \noindent$\blacktriangleright$
\parae{Limited compute.}
Existing SLAM algorithms \textit{cannot run at full frame rate} on mobile computing platforms mounted on drones. A DJI M600Pro (which we use in this paper) hexacopter has a maximum payload weight of 5~kg. It carries an A3Pro flight controller that contains three IMUs and three GNSS receivers. We have also mounted an LTE radio and an Ouster OS1-64 LiDAR, as well as a Jetson TX2 board. This compute capability is far from sufficient to run LiDAR SLAM\footnote{With a 64-beam LiDAR, SLAM processes upto 480 Mbps of 3D data}. 
On the TX2, we ran two popular, representative LiDAR-SLAM algorithms \ie Cartographer~\cite{Cartographer} and LOAM~\cite{zhang2014loam}. \tabref{tab:lidar_slam_compute} shows that Cartographer, a scan-matching algorithm, produces good quality reconstructions, but can only process 2 frames per second (LiDARs generate 20 frames per second). On the other hand, LOAM, a feature-matching algorithm, can process 5 frames per second, but produces poor-quality reconstructions. LOAM fails to track LiDAR frames because the drone's perspective results in sparse features, and poor feature matching. We use Cartographer in this paper.
%\fawad{Added results from running SLAM on a drone}
% \fawad{talk about why we don't use LOAM}
% Lighter weight SLAM algorithms, like LOAM~\cite{zhang2014loam}, that use feature-matching, have lower execution times \ie 200~ms per frame. I However, in our experience, they fail to track the drone's motion because feature matching is not robust enough to handle a drone's challenging view-point.

% \noindent$\blacktriangleright$

\parae{Battery life.}
Drones have \textit{limited flight endurance}. When fully loaded and starting from a full charge, the M600Pro can fly for approximately 25 minutes. This necessitates careful trajectory planning to minimize flight duration.

{\small
\begin{table}
  \centering
  \footnotesize
  \begin{tabular}{|c|c|} \hline
    \textit{\textbf{Challenge}} & \textit{\textbf{Mechanism}} \\ \hline \hline
    Model accuracy & Model collection trajectory planning \\ \hline
    Limited duration & Cheap reconnaissance flight\\ \hline
    Limited compute & Offload compressed point clouds\\ \hline
    Drift accumulation & Flight re-calibration\\ \hline
  \end{tabular}
  \caption{Challenges and contributions}
  \label{tab:challenges}
\end{table}
}

% prior work~\cite{uav_lidar_1,uav_lidar_2} uses \textit{remote sensing} technologies,  specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors and expensive GPS equipment. Both these approaches are compute-intensive and they compute the 3D model \textit{offline} \ie after the drone has landed. 

% What is changing?

%\parab{What have 3D models been used for in the past and how have those models been captured?}
% In general, 3D reconstruction can be useful for a plethora of applications \eg video games, animations in film, as inputs to immersive and virtual reality applications, for architectural planning, to preserve historical sites, to document interior office spaces for construction planning and maintenance, for capturing buildings or rooftops for repair or solar installation \etc. The most dominant approach (\secref{sec:related}) to model collection is \textit{photogrammetry}, a technique which infers 3D models from a sequence of 2D camera images (and the positions associated with these images), captured either using drone-mounted cameras~\cite{7139681, 7989530, 8124461, 8628990} or by humans using ordinary mobile devices~\cite{company_hover}. With the increasing commoditization of LiDAR, 3D model reconstruction can use drone-mounted LiDARs; prior work~\cite{uav_lidar_1,uav_lidar_2} uses \textit{remote sensing} technologies,  specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors and expensive GPS equipment.

% %\parab{Talk about what we can we used 3D models for?}
% Efforts in industry have focused on post-flight integrity assessment of aircraft~\cite{company_austrian_airline}, documenting interior office spaces for construction planning and maintenance~\cite{company_kaarta}, and capturing buildings during construction, or rooftops (for repair, or solar installations)~\cite{company_hover,company_aerial_application,company_drone_deploy}.

% %\parab{How is it collected?}
% The most dominant approach (\secref{sec:related}) to model collection is \textit{photogrammetry}, a technique which infers 3D models from a sequence of 2D camera images (and the positions associated with these images), captured either using drone-mounted cameras~\cite{7139681, 7989530, 8124461, 8628990} or by humans using ordinary mobile devices~\cite{company_hover}. With the increasing commoditization of LiDAR, 3D model reconstruction can use drone-mounted LiDARs; prior work~\cite{uav_lidar_1,uav_lidar_2} uses \textit{remote sensing} technologies,  specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors and expensive GPS equipment. 

% %\parab{How long does it take, and how accurate is it?}
% Most prior research work has explored \textit{offline} reconstruction~\cite{uav_lidar_1,uav_lidar_2,7139681, 7989530, 8124461, 8628990}. They report accuracies in the centimeter to sub-meter range. Industry is starting to use time to model reconstruction as an important market discriminator for brand positioning, promising to deliver models in hours or within a day~\cite{company_drone_deploy}. Only one company we know of so far promises \textit{real-time} reconstruction using a hand-held kit with a stereo camera to reconstruct interior spaces~\cite{company_kaarta}.

% \parab{Our focus.} Motivated by these trends, improvements in 3D sensing, and the increasing  availability of off-the-shelf drones, we focus on \textit{upto sub-meter accurate, autonomous, real-time reconstruction of large buildings} using a drone-mounted LiDAR. Unlike the hand-held kit developed by~\cite{company_kaarta} which requires a human-in-the-loop to navigate the interior space, we aim to develop a completely automated solution given only an approximate location of the building(s) to reconstruct. To achieve the three requirements \ie accuracy, autonomy and real-time 3D reconstruction, our approach devises algorithms to reconnoiter the specified area, then designs a trajectory to obtain the 3D model. However, these tasks are challenging for the following reasons. To achieve sub-meter accuracy, to position 3D point clouds, we cannot use GPS (because it is inaccurate), so we must use Simultaneous Localization and Mapping (SLAM~\cite{slam_part1})\footnote{Two startups we know of~\cite{hovermap, Prometheus} also use SLAM for drone \textit{offline} reconstruction (\secref{sec:related}).}. technologies. However using SLAM on a drone is particularly challenging because: a) relative to vehicle SLAM, on a drone, SLAM algorithms have access to 10~x sparser point clouds, b) at the same time, model collection must be relatively fast because of a drone's limited battery life, and c) both these can result in significant drift error accumulation, inherent to SLAM algorithms. To achieve autonomous reconstruction, identifying the exact location and boundary of the building can be challenging due to the large variety of building shapes and nearby objects like trees \etc. Lastly, to enable real-time reconstruction, processing point clouds can require compute resources well beyond those on today's drones.

% This is challenging because there are multiple dimensions that a solution must reason about: drone battery, the height, speed and orientation,

% The increasing availability of off-the-shelf drones has democratized 3D modeling. Today, to build a 3D model, a human operator can draw a trajectory for the drone on an app (\eg the DroneDeploy app~\cite{dronedeploy}). To do this, the operator relies on area surveys from secondary sources, such as satellite imagery, to define trajectory. The drone follows this trajectory while continuously capturing sensor imagery. When it lands, the operator offloads sensor data directly from the UAV to a ground station, that will then execute the 3D processing pipeline. The resulting 3D model must be manually inspected for completeness and correctness, and a new data capture flight must be conducted if it: a) does not capture points of interest (\eg buildings) or, b) fails (either completely or partially). This is repeated as many times as necessary to construct a good 3D model.

% Removing the human-in-the-loop and automating most steps in 3D reconstruction can significantly improve the speed and accuracy of 3D model generation. To this end, in this paper we ask: Given only a coarse location of a building, can we \textit{reconstruct a 3-D model} of a building to \textit{sub-meter accuracy} in \textit{near real-time} (\ie the reconstruction completes before the drone flight finishes) using only off-the-shelf drones and sensors? Near-real time reconstruction can be important during disaster response, or for continuously updated digital 3D reconstruction during construction. More generally, however, this aggressive goal can expose opportunities for new applications as well as systems bottlenecks.

% \parab{Challenges.} Drones are limited in the weight of the payload they can support, and the distance they can fly on a single charge (\secref{s:challenges}). 3D reconstruction requires a sensor capable of depth perception; in this paper, we consider a drone-mounted LiDAR. A LiDAR can add significant weight to the drone, so careful trajectory planning is essential to achieve our goal of accurate reconstruction. Drones can carry GPS receivers, but positioning error from commodity GPS receivers can be several meters, especially in obstructed environments. Low positioning error is crucial to achieving sub-meter accuracy. Simultaneous mapping and localization (SLAM~\cite{slam_part1}) technologies can provide accurate positioning, but SLAM can be sensitive to flight parameters and incur drift (\secref{s:challenges}). Finally, SLAM, as well as 3-D reconstruction itself are significantly compute-intensive and require server-class hardware for real-time processing; such hardware cannot be mounted on the drone. Offloading these to the cloud is challenging because depth perception sensors like LiDARs can generate significant amounts of raw data (a few hundred Mbps).

%% To this end, we ask ourselves the following question: how can we \textit{automate} data-collection from the drone so that it is a single-time process. We believe a promising direction for this is to remove the human-in-the-loop and use a control-feedback loop. In this approach, the drone initially flies in a predetermined trajectory during which it perceives the environment using a depth perception sensor. While doing this, the drone continuously sends 3D data to a cloud service in real-time. The cloud service uses this data to understand the underlying environment and evaluate the quality of the 3D model instantly. Based on this understanding and the 3D model, the cloud service tells the drone how and where to scan by adjusting its trajectory and flight parameters (\eg speed, altitude \etc).

%% The key challenges in this approach are to find imperfections in the 3D model and objects of interest in the underlying environment in near real-time to adapt the flight of the drone accordingly.

% \fawad{The three challenges in order of difficulty are are: accuracy, autonomy, and real-time. Trajectory planning takes care of accuracy. Recon phase takes care of autonomy whereas system design takes care of real-time.}

\parab{Contributions.} This paper presents the design and implementation of a system called \sysname, which makes the following contributions to address these challenges (\tabref{tab:challenges}).

\parae{Model collection trajectories.} \sysname's first contribution is the design of \textit{model collection trajectories} that navigate the competing constraints \ie accuracy and battery life (\secref{s:slam-phase}). Model collection uses SLAM, and SLAM error is sensitive to how the LiDAR is mounted, how fast and at what height the drone flies. Faster, higher flights use less of the drone's battery, but can incur high SLAM error. The converse is true of slower and lower flights. \sysname finds a sweet spot in this trade-off space to balance its accuracy goals with drone battery usage. Even so, SLAM can incur \textit{drift} on longer flights. 
%As such, even with well-designed trajectories, LiDAR-based \textit{offline} reconstruction cannot neutralize \textit{drift} errors (as we show in \secref{sec:eval:accuracy}). 
\sysname needs to detect excessive drift for which it uses a novel algorithm that tracks consistency between \textit{the shape of} GPS traces and SLAM positions to detect excessive drift, then incorporates a \textit{re-calibration} step to correct for it while the drone is \textit{in-flight}.

\parae{Reconnaissance flight.} \sysname's efficient model collection trajectories, scans over large areas can exhaust a drone's battery. To this end, \sysname's second contribution is a robust and efficient \textit{geometry extraction} algorithm (\secref{s:area-inter-reconn}) that helps \textit{focus model collection} only on the structure\footnote{In this paper, we focus on extracting the boundary of a building and leave generalization to future work} to reconstruct. This algorithm, which runs during a \textit{reconnaissance flight} before model collection, works well even with a fast, high flight that minimizes drone flight duration (and hence battery usage). During the flight, this algorithm extracts the building geometry without constructing the 3D model; it relies on detecting planar surfaces by using the consistency of surface normals across points on a plane, then estimates building height and boundary from the plane forming the rooftop. \sysname uses this boundary to plan the \textit{model collection trajectories} described above.

\parae{Cloud offload.} \sysname's third contribution is the design of a processing pipeline that (a) offloads computation to a cloud server by compressing point clouds on the drone to the point where they can be transmitted over LTE (\secref{s:compression}), and (b) that leverages GPU acceleration to process these point clouds in near real time at the LiDAR frame rate and with minimal end to end processing delay (\secref{sec:eval}).

% architected as follows: Given a rectangular region that encompasses a building, a cloud-based service generates energy-efficient drone trajectories to find the building and collect its 3D model. As the drone flies, it streams compressed LiDAR data over LTE; the cloud service runs SLAM in near real-time, adjusts the trajectory to minimize drift, and reconstructs the 3D model on the fly (\secref{sec:design}). To minimize drone battery usage, \sysname conducts a fast, energy-efficient \textit{reconnaissance} flight to determine the boundaries of the building, then runs a slower \textit{model collection} flight within the building's boundaries that carefully balances drone battery usage while ensuring high reconstruction accuracy. To achieve this, \sysname makes three contributions.

% Its third contribution is the design of a software pipeline, leveraging GPU acceleration, that ensures that these algorithms can run on the cloud in near real-time (\ie at the frame rate of the LiDAR), and with minimal end-to-end processing delays (\secref{sec:eval}).

Experiments (\secref{sec:eval}) on real-world drone flights and a photo-realistic drone simulator (AirSim~\cite{airsim}) demonstrate that \sysname can achieve 21-30~cm reconstruction accuracy even after compressing the raw sensor data by almost two orders of magnitude. Not only is \sysname \textit{faster} than a state-of-the-art photogrammetry approach~\cite{colmap}, it is also \textit{more accurate}, since the latter cannot re-calibrate mid-flight. %\fawad{Added the top sentence.}
An experiment using the complete \sysname implementation is able to stream compressed point clouds over LTE, reconstruct the 3D model on-the-fly and deliver an accurate 3D model about 100~ms after flight completion. \sysname's choice of trajectories drains the battery least while achieving the accuracy target, and its pipeline can process frames at 20~fps while incurring a processing latency of less than 100~ms. To our knowledge, \sysname is the first to demonstrate on-line, cloud-based, autonomous, sub-meter, 3D model reconstruction.

% \fawad{Added text about \sysname being faster and more accurate than photogrammetry}

% %% Our first contribution is an efficient imperfection detection module that runs at the cloud in near real-time. Pipelines for building and comparing 3D models are computationally and time intensive. Such pipelines are infeasible in our application because they cannot provide quick feedback to the drone during flight. We show that is possible to quickly infer imperfections in the 3D model without computing the whole model. To do this, we run half of the 3D reconstruction pipeline and compare its intermediate product with cues from other on-board drone sensors like GPS.

% %% The imperfection detection module identifies regions of poor reconstruction, however, to capture objects of interest, the drone needs an understanding of the underlying scene. Deep learning models for object detection exist for ground vehicles like cars but, to the best of our knowledge, there are no models for drones. To this end, our second contribution is an efficient and robust detection module that locates objects (e.g., buildings, cars, etc) of interest in the environment. To ensure the drone can use this understanding during flight, we use raw output from the 3D sensors instead of the processed 3D model to detect objects.

% %% To complete the control feedback loop, the drone must use the two sets of feedback about imperfections and objects of interest to reconstruct better by adapting its trajectory in real-time. To this end, our third contribution is a path-planning algorithm that uses feedback from the cloud and the drone’s flight log. This algorithm computes a path for the drone by prioritizing different regions for exploration and re-exploration based on the drone’s remaining battery life.

% %% During the data collection phase, the drone collects both good and bad 3D sensor data. Our final contribution is an algorithm that intelligently selects a subset of the sensor data for accurate 3D reconstruction.

% %% We embody these contributions in the form of a system called \sysname.


% \section{Background}
% \label{sec:motivation}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\columnwidth]{figs/lidar_spec}
% %     \caption{LiDAR scanning has a vertical and horizontal coverage. 
% %         \label{fig:lidar_spec}}
% % \end{figure}
% %% \ramesh{We'll need some background on UAVs, with particular attention to what
% %% hardware these have: compute, LTE, GPS, LiDAR. Also weight constraints. Perhaps
% %% add a picture of the NEC drone?}

% %\eugene{Some of these details can go into the evaluation section instead.}

% %% \begin{figure}
% %%     \centering
% %%     \includegraphics[width=0.8\columnwidth]{figs/coverage_distance}
% %%     \caption{Ouster OS1-64 LiDAR  horizontal and vertical coverage 
% %%         distances at different drone
% %%         altitudes.\label{fig:lidar_coverage}}
% %% \end{figure}
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.8\columnwidth]{figs/drone-old}
% %     \caption{Early prototype of the \system drone. \system is migrated to a M600Pro for this work.}
% %     \label{fig:drone}
% % \end{figure}



% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\columnwidth]{figs/fig_tx2_ransac.pdf}
%   \caption{Plane-fitting on an nVidia TX2 \label{fig:tx2_plane_fitting}}
% \end{figure}

% \parab{The challenges.}
% 3D model collection from aerial drones is particularly challenging due to two competing constraints (accuracy and battery-life). Unlike ground robots like vehicles, on an aerial drone, LiDAR SLAM algorithms have access to only 9\% of the entire point cloud (because the drone is in the air). To compensate for this, drones can fly slow and close to the building for better positioning. However, this is not possible because of a drone's limited battery life. \sysname tackles this challenge on two fronts: a) it uses an offline parameter study and a real-time recalibration module to reduce positioning error, and b) it collects the 3D model in two steps \ie a fast reconnaissance phase to identify the region of interest and a slower data collection flight to collect the actual 3D model.

% A strawman solution to our problem of real-time model collection is to execute LiDAR data processing and model construction entirely on the drone. This is not likely to be feasible anytime in the near future. To demonstrate this, we ran a standard plane-fitting algorithm~\cite{ransac} on a single Ouster LiDAR point cloud; plane-fitting is a primitive we use in \secref{sec:design} to detect the rooftop of the building. On our drone's TX2, this operation can take nearly 0.5~s~ (\figref{fig:tx2_plane_fitting}) on a single point cloud, on average. Our LiDAR generates 20 point clouds every second, and plane-fitting is only one of the many expensive operations we require (\secref{sec:eval}). To put this in perspective, the plane-fitting algorithm contributes 5\% to the execution time of the entire pipeline. This means, if we ran \system on the drone, it would process a single second's data in 200 seconds.

% For this reason, \sysname \textit{offloads} most computation to the cloud (\figref{fig:overview}). The drone obtains point clouds from the LiDAR, compresses them, and streams the point clouds to a cloud VM that performs near real-time 3D model construction.



% % \ramesh{Fawad: Let's run ransac/surface normals on 100 point clouds from real data and report the CDF?}
% % \fawad{Ramesh: added the figure here}

% % Fig.~\ref{fig:drone} shows an early prototype of the \system on a DJI Wind 4. The \system payload is mounted onto a M600Pro for real-world experiments in this paper.

% %\ramesh{I removed the drone photo. If we can't get the photo of the one we used, let's not put an alternative, since this begs the question: why not a photo of the original?}

% % Relevant to this paper is the drone battery consumption for different kinds of flight. Unfortunately, this depends significantly on the drone weight and payload. For our drone platform, we have measured battery depletion for horizontal and vertical flights as a function of speed and height. Because our drone is heavy and carries a maximal payload, our measurements indicate that: (a) vertical and horizontal flights drain the battery at roughly the same rate (0.065\% per second of flight), and (b) speed and height do not significantly affect battery drain. This simple model drives the design of drone trajectories (\secref{sec:design}) and we have left it to future work to explore more sophisticated models.

% % The other aspect that impacts drone battery drain is the interplay between LiDAR geometry and the drone height. Intuitively, the higher the drone flies, the more the LiDAR ground coverage, so the shorter the flight can be, but the less resolution in the resulting data (LiDAR beams are radial, so points farther away have lower resolution). Navigating this tension is one of the central challenges in our paper.

% %% \figref{fig:lidar_orientation} illustrates the mounting position of the LiDAR on
% %% the \system UAV.  \figref{fig:lidar_orientation} also shows the horizontal and
% %% vertical coverage distance of the LiDAR. This refers to the horizontal and
% %% vertical ground distance (w.r.t.  the LiDAR) of the intersection between the
% %% field of view of the LiDAR and the ground. Objects within this coverage region
% %% will be scanned and captured in the point cloud returned by the LiDAR sensor.
% %% \system uses an Ouster OS1-64 LiDAR
% %% and its horizontal and vertical distances w.r.t. the altitude of the UAV above
% %% the ground is shown in \figref{fig:lidar_coverage}.



% %% \begin{figure}
% %%     \centering
% %%     \includegraphics[width=0.8\columnwidth]{figs/coverage_distance}
% %%     \caption{Ouster OS1-64 LiDAR  horizontal and vertical coverage 
% %%         distances at different UAV
% %%         altitudes.\label{fig:lidar_coverage}}
% %% \end{figure}


% %% \parab{LiDAR Orientation.} \system uses two LiDAR orientations, as shown in
% %% Fig.~\ref{fig:lidar_orientation}: parallel and perpendicular.  In the
% %% \emph{parallel (perpendicular)} orientation, the scan plane of the LiDAR is
% %% parallel (perpendicular) to the direction of flight.
% % \subsection{Challenges}
% % \label{s:challenges}
% % \parab{A strawman approach.} To motivate the challenges described in the paper, consider the following strawman solution. A user wishing to obtain a 3D model (a) locates the target building on a map, (b) estimates the contours of the building, (c) plans the flight path of the UAV to collect point-clouds of the building, and (d) at the end of the flight aggregates the collected point-clouds, together with the point-cloud positions. The resulting collection of \textit{oriented point-clouds} constitutes the 3D model of the building.

% % \parab{Real-time automated 3D modeling.} \sysname automates all of these steps, given \textit{only} a rectangular region containing the building. It makes the 3D model of the building available \textit{even before the UAV completes its flight}. This motivates algorithmic and systems challenges.

% % \parae{Algorithmic challenges.} How can the UAV recognize the contours of the building in real-time? The most robust solution to this approach would rely only on the UAV's sensory inputs, rather than additional sources such as maps \etc In this case, the challenge becomes: How can the UAV efficiently detect the contours of the building from LiDAR scans?

% % Step (d) above motivates the second algorithmic challenge. In that step, constructing a 3D model requires the precise \textit{pose} (position and orientation) of each point cloud. In theory, the GPS reading, together with inertial measurements, can provide point cloud poses. However, low-cost, lightweight GPS receivers can, in urban environments, exhibit high error. Remote sensing approaches use high-precision GNSS/RTK receivers that are difficult to deploy and use in urban environments due to the multiple obstructions that degrade accuracy (\eg prior work~\cite{Carloc} reports RTK-enabled receivers can exhibits tens of meters error in downtown environments). Hence, a solution to this problem of determining pose must rely pre-dominantly on sensors onboard the UAV.

% % We observe that LiDAR SLAM (Simultaneous Localization And
% % Mapping~\cite{slam_part1, slam_part2}) algorithms can provide accurate pose
% % estimates. These algorithms use scan or feature matching techniques to align
% % consecutive LiDAR frames to determine the pose of the UAV throughout its flight.
% % Both these methods compare overlapping regions of two LiDAR frames to determine
% % their relative pose. The Iterative Closest Point (ICP)~\cite{icp} algorithm is a
% % well-known technique for this scan matching. Given two LiDAR frames $\mathbf{A}$
% % and $\mathbf{B}$, ICP finds the closest match from each point in the source
% % point cloud $\mathbf{A}$ to a point in the reference point cloud $\mathbf{B}$.
% % It then estimates the transformation (translation and rotation) that will best
% % align each point in $\mathbf{A}$ to its corresponding point in $\mathbf{B}$. ICP
% % applies this transformation to $\mathbf{A}$ and repeats until the matching
% % error falls below a specified threshold. The consecutive poses of all LiDAR
% % frames collectively form the SLAM trajectory of the UAV along its flight
% % relative to the first LiDAR frame.

% % SLAM algorithms can accumulate positional \textit{drift}. They use techniques
% % like \textit{loop closure} (recognizing when a previously visited location is
% % re-visited) to mitigate drift. Even so, over longer flights, drift can
% % accumulate, so a second set of algorithmic challenges \sysname faces is: (a) how
% % to detect when the UAV has accumulated excessive drift? and (b) how to
% % \textit{re-calibrate} the UAV once it has detected excessive drift?  

% % \parae{Systems challenges.} For weight and cost reasons, UAVs have minimal on-board compute and storage. The \system UAV can only carry 5kg of payload, hence it is limited to a low-powered, mobile dual core Intel i7 system to allow the battery and LiDAR to also be carried safely. With these resources, running a LiDAR SLAM algorithm is simply infeasible. At the same time, it is difficult to \textit{offload} this computation, since LiDAR point-clouds are voluminous: uncompressed point clouds from a 64-beam LiDAR require hundreds of Mbps over the LTE connection.

% %\ramesh{Let's discuss how best to plug two holes in the story: why is real-time reconstruction important? why not use high-end GPS+Inertial boxes?}

% %% \subsection{3D Reconstruction Pipeline} 

% %% A 3D reconstruction pipeline consists of three main steps: (a) estimating the 3D
% %% pose (i.e. trajectory and rotation) using 3D Simultaneous Localization And
% %% Mapping (SLAM)~\cite{slam_part1, slam_part2} on the incoming LiDAR data stream;
% %% (b) translating the rotating each LiDAR frame to match its predicted post; and
% %% (c) appending all the transformed LiDAR point clouds to form the complete 3D
% %% model.

% % \system builds a 3D model $D$ in three steps: a) estimate the 3D pose $t_i$
% % (translation and rotation) of the drone for each point cloud $p_i$, b) transform
% % the point cloud to its predicted pose, and c) append all transformed point
% % clouds. 
% % 
% % \begin{equation}
% % \label{equation:reconstruction}
% %     D = \sum_{i=0}^{n} ( t_i * p_i )
% % \end{equation}
% % 
% % Given \eqref{equation:reconstruction}, if we assume LiDAR point clouds are accurate by 
% % flying less than 120m (range of LiDAR~\cite{Ouster}) from the ground plane, 
% % the only source of error stems from pose estimation of the drone. To do this accurately, \
% % system uses a LiDAR SLAM algorithm (Google Cartographer)~\cite{GoogleCartographer}.

% %% \parab{3D SLAM} uses scan, or feature matching techniques to align consecutive
% %% LiDAR frames to determine the pose of the UAV throughout its flight. Both these
% %% methods compare overlapping regions of two LiDAR frames to determine their
% %% relative pose. The Iterative Closest Point (ICP)~\cite{icp} algorithm is a
% %% well-known technique for scan matching. Given two LiDAR frames $\mathbf{A}$ and
% %% $\mathbf{B}$, ICP finds the closest match from each point in the source point
% %% cloud $\mathbf{A}$ to a point in the reference point cloud $\mathbf{B}$. It then
% %% estimates the transformation (translation and rotation) that will best align
% %% each point in $\mathbf{A}$ to its corresponding point in $\mathbf{B}$. This
% %% transformation is applied to $\mathbf{A}$ and the process is repeated (\ie
% %% iterated) until the matching error falls below a specified threshold.  The
% %% consecutive poses of all LiDAR frames collectively form the SLAM trajectory of
% %% the UAV along its flight w.r.t. the very first LiDAR frame.

% %% The accuracy of scan matching two LiDAR frames is dependent 
% %% on the amount of overlap between the frames: the greater the 
% %% number of common points between the frames, the better 
% %% the scan matching algorithm can align them. 

% %% \cm{Need RMSE graphs with UAV at different speeds. Orientation is not important
% %% here}

% %% \parab{3D Reconstruction} takes place after the pose of each LiDAR frame is
% %% estimated by scan matching. \system translates and/or rotates each LiDAR frame
% %% according to its associated pose, and appends the LiDAR frame with all previous
% %% frames to build up a 3D model of the area scanned by the LiDAR. Note that each
% %% new LiDAR frame has an overlap with previous frames.  The \emph{density} of the
% %% final 3D model is dependent on this overlap: a slow UAV flight velocity
% %% resulting in a large overlap between consecutive LiDAR frames will generate a 3D
% %% model of high density.  And the higher the model density, the greater its
% %% fidelity and accuracy (i.e. greater ability to capture smaller features in the
% %% area).  The goal of \system is to attain the greatest possible model accuracy,
% %% while respecting the LiDAR characteristics and flight endurance of the UAV
% %% platform.


% % SLAM aligns consecutive scans and uses the alignment information to estimate the
% % pose of the drone. To align scans, SLAM use scan matching, and feature matching
% % techniques. Hence, the accuracy of pose estimation (and the 3D model) directly
% % depends on the ability of SLAM to accurately align multiple point clouds.  We
% % performed an exhaustive study of flight parameters like speed, height, and
% % orientation of the LiDAR using real-world traces as well as synthetic traces
% % from Airsim~\cite{Airsim} to study their effects on the accuracy of SLAM pose
% % estimation.

% % Here we should add graphs that show how 3D model RMSE responds to changes in
% % speed, orientation, and height of the drone

% % \begin{figure}
% %     \label{fig:airsim_height_vs_rmse}
% %     \centering
% %     \includegraphics[width=\columnwidth]{figs/airsim_height_vs_rmse.pdf}
% %     \caption{Flying the drone close to the building, and use a parallel 
% %     orientation of the LiDAR yields more accurate 3D models.}
% % \end{figure}
% % 
% % \begin{figure}
% %     \label{fig:airsim_speed_vs_rmse}
% %     \centering
% %     \includegraphics[width=\columnwidth]{figs/airsim_speed_vs_rmse.pdf}
% %     \caption{With a parallel orientation of the LiDAR, the drone 
% %     can fly faster and get good reconstruction quality.}
% % \end{figure}

% % \begin{figure}
% %     \label{fig:real_speed_vs_rmse}
% % \end{figure}
% % 
% % \begin{figure}
% %     \label{fig:real_height_vs_rmse}
% % \end{figure}

% % On the drone, there are two orientations of the LiDAR \ie parallel, and perpendicular
% % as shown in \figref{fig:lidar_orientation}. When the LiDAR is parallel to the direction 
% % of motion, there is a larger common area between consecutive point clouds and hence it is 
% % easier to align point clouds. On the other hand, in the perpendicular orientation, the common 
% % scan area between consecutive point clouds is smaller. As a result, the reconstruction errors 
% % for parallel orientation are relatively smaller even at higher speeds of the drone 
% % \figref{fig:airsim_speed_vs_rmse}, \figref{fig:real_speed_vs_rmse}.
% % 
% % Although as the drone moves higher LiDAR coverage area increases, the point resolution 
% % of the point cloud decreases \figref{fig:lidar_coverage}. As a result, SLAM cannot match 
% % consecutive point clouds and this result holds for both parallel, and perpendicular 
% % orientations of the LiDAR \figref{fig:airsim_height_vs_rmse}, \figref{fig:real_height_vs_rmse}.





==> intro.tex <==
\section{Introduction}
\label{sec:intro}
% The quality of a 3D model depends on two metrics: accuracy and completeness. Accuracy represents \textit{how well} a reconstruction resembles the real-world object. Completeness represents \textit{how much} of real-world object the reconstruction contains (discussed in detail later).

% Drone based 3D reconstruction
\parab{Drone-based 3D reconstruction.}
In recent years, with the commoditization of drones, they can be equipped with on-board compute, cellular radios (LTE) and sophisticated sensors like stereo cameras, and LiDARs\add{,} \etc
% The last few years have seen impressive advances in the commoditization of drones. Today, drones can be equipped with on board compute, a cellular (LTE) radio and sophisticated sensors (\eg cameras, stereo cameras and LiDAR). 
Given this, in the coming years, drones will likely revolutionize aerial photography, mapping and three-dimensional (3D) reconstruction. 
Recent estimates put the total market for drone-based \textit{3D reconstruction}, the task of generating a digital \textit{3D model} of the environment, at 21 billion US dollars by 2025~\cite{drone-market-1, drone-market-2}.
% \raj{Comma before \etc}

% What is a 3D Model
\parab{What is a 3D model?}
The term \textit{3D model} covers a range of geometric representations of the surfaces of objects, from coarse-grained approximations (cylinders, cubes, intersection of planes), to more \add{fine-grained} representations such as \textit{meshes} (small-scale surface tessellations that capture structural variations). In this paper, we seek to extract a \add{fine-grained} \textit{point-cloud} of a large structure (\eg a building) which consists of dense \textit{points} on the surface of the structure. Each point has an associated 3D position, along with other attributes (depending on the sensor used to generate the point-cloud). A point-cloud based 3D model can generate all other representations.
% \raj{Either we can write "coarse-grained" and "fine-grained", or "coarse-grain" and "fine-grain" in above paragraph}

%In this paper, we focus on reconstructing the 3D model of large structures specifically buildings\footnote{Though our evaluations mostly focus on buildings, we show (\secref{sec:eval}) that \sysname can generalise and be used for other large structures \eg blimps as well}.

% What have been the applications of 3D models in the past?
\fawad{The following paragraph can go.}
\parab{Applications.}
3D models are used in animations in films and video games, for preserving historical and tourist sites, for archaeology, city planning, and to capture buildings or rooftops for repair and solar installation, and as inputs to immersive virtual reality (VR) applications. Recently, startups are promising to deliver models in hours or within a day~\cite{company_drone_deploy} after drone data collection. This trend has inspired newer, more time-sensitive applications of 3D modeling such as construction site monitoring~\cite{company_drone_deploy}, damage assessment~\cite{drone_disaster_relief_1, drone_disaster_relief_2, drone_disaster_relief_3, company_austrian_airline},
and documenting interior office spaces~\cite{company_kaarta}.
\raj{Structure the first sentence: "from archaeology, city planning to capture buildings or rooftops ..."}

% like (a) post-disaster reconstruction for search and rescue missions~\cite{drone_disaster_relief_1, drone_disaster_relief_2, drone_disaster_relief_3, drone_disaster_relief_4, drone_disaster_relief_5}, (b) construction site monitoring~\cite{company_drone_deploy}, (c) mapping mines, cell-towers and tunnels~\cite{hovermap, Prometheus}, (d) documenting interior office spaces~\cite{company_kaarta}, (e) inspecting oil and gas installations~\cite{drone_oil_gas}, and (f) between-flight modeling of aircraft fuselages or blimps to determine structural integrity~\cite{company_austrian_airline}.

\parab{State-of-the-art: Photogrammetry.}
% \todo{think abt adding NERF here because it properties i.e., complexity and need for good data collection, are similar to photogrammetry.}
Today, to build a 3D model, a drone operator flies a drone around a physical structure in a given trajectory to collect 2D images. 
After the drone lands, the operator uploads these images to a cloud service. 
The cloud service uses \textit{photogrammetry} to build a 3D model. 
\textit{Photogrammetry} (\secref{sec:related}) infers a 3D model from a sequence of 2D images captured using drone-mounted cameras~\cite{7139681, 7989530, company_hover}, and is \textit{computationally intensive}. 
The quality of the inferred models depends on the quality of the 2D images, which \textit{depends on the drone's flight trajectory}. 
To obtain accurate reconstruction, photogrammetry can require multiple iterations with human-intervention for trajectory design. We quantify these shortcomings of photogrammetry in \secref{sec:background_motivation}.

% If the drone flies too fast, for instance, the inferred 3D model will contain missing regions, requiring a human operator to redesign the trajectory and fly the drone again~\cite{mvslessons, photogrammetryissues}. The iterative approach, together with the fact that photogrammetry is expensive, means it can take several hours to days to obtain a 3D model.

% After 3D reconstruction, the operator \textit{manually} inspects the 3D model's quality.
% % or by humans using ordinary mobile devices~\cite{company_hover}. 
% % Photogrammetry \textit{infers} 3D models using a technique known as multi-view stereo~\cite{furukawa15:_multi_view_stereo}, 
% % These algorithms combine information from successive images, together with information about local motion, and inferred camera parameters such as the focal length. 
% % \parab{Problems with photogrammetry.}
% If the model is not visually pleasing, the operator adjusts the trajectory, flies the drone, and reconstructs the 3D model.
% % Photogrammetry is computationally exp
% % The 3D model's quality depends on the drone's trajectory
% The quality of the 3D model depends on trajectory design but there are no established rules for trajectory design.
% Moreover, photogrammetry is computationlly expensive, so it can take several days to complete the entire 3D reconstruction process.
% % In photogrammetry, the quality of the reconstructed 3D model depends on the trajectory used to capture the physical structure.
% % If not carefully crafted, the quality of the 3D model is poor.
% % resulting 3D model is \textit{incomplete} and contains \textit{missing} regions.
% % This visual inspection is manual.
% % When this happens, the operator adjusts the trajectory, flies the drone, and reconstructs the 3D model again~\cite{mvslessons, photogrammetryissues}.
% % Because there are no established rules for trajectory design~\cite{mvslessons, photogrammetryissues}, it can take multiple iterations to get the desired 3D model.
% % Moreover, photogrammetry approaches estimate depth from 2D images, their reconstruction times are relatively large \ie from several hours to days~\cite{company_drone_deploy} for large structures.
% % Photogrammetry is slow, so it can take several days to complete the entire 3D reconstruction process.
% In theory, photogrammetry can avoid this iterative approach if it could detect, in-flight, when the model might be incomplete and adapt the trajectory accordingly. 
% This has proven to be hard to do without running the entire photogrammetry pipeline~\cite{mostegel2016uav, 7422384} on the set of images.

\parab{Drone-mounted LiDAR-based reconstruction.}
Unlike photogrammetry, LiDAR-based reconstruction can more directly infer 3D models, because LiDARs directly provide depth information (unlike cameras). A LiDAR sensor measures distances to surfaces using lasers mounted on a mechanical rotating platform. With each revolution of the lasers, the sensor returns a point cloud, or a \textit{LiDAR frame}. The point cloud is a set of 3D data points, each corresponding to a distance measurement of a particular position of the surrounding environment from the LiDAR. For instance, an Ouster OS1-64 LiDAR~\cite{ouster_guide} has 64 lasers that scan at 10 to 20~Hz, with a horizontal and vertical field of view of 360$\degree$ and 45$\degree$, respectively.

To reconstruct a structure such as a building, one can mount a LiDAR on a drone, fly the drone around the building, and \textit{merge} points clouds captured from different locations around the building. Consider point clouds $p$ and $p'$. A point $x$ on the surface of the building may appear both in $p$ and $p'$. However, since the drone has moved, this point $x$ appears at different positions (relative to the LiDAR) in the two point clouds. If we precisely transform both point clouds to the same coordinate frame of reference, then the union of points in $p$ and $p'$ constitutes part of the 3D model of the building. This operation is fast, but \textit{depends critically on knowing the precise pose (orientation and position) of the drone} when it captures point clouds.

\parab{SLAM for positioning.} LiDAR SLAM (Simultaneous Localization and Mapping~\cite{slam_part1, slam_part2}) algorithms can provide accurate \textit{pose} estimates,\footnote{In \secref{sec:background_motivation}, we explain why other approaches (\eg using GPS or GNSS/RTK) can be inaccurate.} which can be used to position point clouds. These algorithms use scan~\cite{Cartographer} or feature matching~\cite{zhang2014loam, liosam} techniques to align consecutive point clouds to determine the pose of the drone throughout its flight.

% , a topic which will be discussed in more detail in the following section. 

\parab{Challenges.}
Although SLAM is used for precise positioning in autonomous driving, it presents three distinct challenges when mounted on a drone (quantified in \secref{sec:background_motivation}).

\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,leftmargin=*]
% \item 
% The core challenge in this paper is to use SLAM for precise positioning on a drone.
% \item Point clouds captured from a drone are significantly sparse relative to ones captured from a vehicle \ie a drone captured 3D point cloud has less than 1/10th of the 3D points as compared to ones captured from a vehicle (\figref{fig:slam_challenge}).

\item Drones capture significantly sparser point clouds (with less than 10\% of 3D points) relative to those captured by vehicles (\figref{fig:slam_challenge}).
SLAM fails to accurately align sparse point clouds, resulting in imprecise pose estimates.
For precise positioning, SLAM needs careful flight trajectory planning, \eg flying fast results in low overlap and hence inaccurate alignment. \raj{also add that flying too slow increases flight time.}
% If the drone flies too fast, for example, successive point clouds may not overlap enough to effect good alignment.
% This necessities slow and long flights but a drone has a limited battery life.
% An industrial grade drone, the DJI M600Pro (used in this paper), can fly for only 25 minutes on a full charge.
As such, \textit{the core challenge in this paper is to design a flight trajectory that ensures accurate SLAM positioning}.

% The drone's flight trajectory, parameters, and the orientation of the LiDAR on the critically impact SLAM's ability to align point clouds. 
% SLAM estimates positions by aligning successive point clouds, and alignment relies on the overlap between point clouds. 

% As such, 

\item Although accurate positioning needs careful trajectory with slow and long flights, drones have limited battery lives.
An industrial grade drone, the DJI M600Pro (used in this paper), can fly for approximately 25 minutes.
This requires trajectory planning that ensures both high positioning accuracy and low flight duration.

% \item Even with a well-designed trajectory, SLAM \textit{accumulate drift}~\cite{slam_part1,slam_part2}, so position estimates can degrade on longer flights.

\item Besides this, drones can carry a limited payload, restricting the amount of compute power they can carry.
However, existing SLAM algorithms \textit{cannot run at full frame rate} on these mobile computing platforms.
% Because of this, existing SLAM algorithms \textit{cannot run at full frame rate} on mobile computing platforms mounted on commodity drones.
% Detecting and correcting for this drift mid-flight can avoid re-doing the entire flight (as may be required for photogrammetry). 


% \item Drones have limited flight endurance. When fully loaded and starting from a full charge, an industrial grade DJI M600Pro drone can fly for approximately 25 minutes. This necessitates careful trajectory planning to minimize flight duration.
\end{itemize}

% \fawad{see if we can add point density in the mix somewhere}


% leveraging it for precise positioning on a drone presents a major challenge.  
% As such, the core challenge in this paper to use LiDAR S

% A LiDAR SLAM-based 3D reconstruction approach presents four distinct challenges (quantified in \secref{sec:motivation}):


\parab{Our contributions.} This paper presents the design and implementation of \sysname, which quickly builds high-quality 3D models of large physical structures, which, unlike photogrammetry, is \textit{computationally-efficient} and does not require \textit{iterative capture} or \textit{human-intervention}. \sysname consists of a lightweight module that streams 3D point clouds from the drone to a powerful cloud-based module which performs more computationally-intensive tasks.


To address the challenges described above, \sysname makes three contributions (\tabref{tab:challenges}):

\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,leftmargin=*]

% Before
% \item The core contribution of this paper is a novel optimization formulation to obtain 3D flight trajectories that capture point clouds of large buildings whilst: a) maximizing SLAM positioning accuracy, b) minimizing flight duration, and c) capturing the given 3D model at a user-defined point density.
% Point density, the number of points per unit area on the reconstructed 3D model, allows users to define the detail at which to capture 3D models.
% % Point density is the number of points per unit area on the reconstructed 3D model. 
% % This knob allows users to define the detail at which to capture 3D models.
% % \footnote{Level of detail refers to the point density of the point cloud. The point density is the number of points per unit area on the reconstructed 3D model. This knobs allows users to define the detail at which to capture the 3D model.} 
% % \textit{The core contribution of this paper is a set of techniques that define \textit{how to fly} the drone to maximize accuracy and minimize energy consumption.
% % \sysname uses a novel optimization formulation to obtain minimal duration 3D flight trajectories to capture 3D point clouds of a large class of buildings (encompassing more than 99\% of buildings across several cities (\secref{sec:design})).
% % To do this, \sysname uses an exhaustive parameter search to find optimal flight parameters, an analytical model to determines effective point cloud regions for the density constraint, and uses
% % To do this, \sysname uses exhaustive parameter search for flight parameters, an analytical LiDAR model for  and an ILP-based optimization process (\secref{s:slam-phase}).
% To do this, \sysname performs an exhaustive parameter search to find optimal flight parameters that minimize positioning error.
% Then, whilst capturing the 3D model with those flight parameters, it determines the effective region of the LiDAR point cloud which satisfies the point density constraint. 
% Finally, \sysname uses an Integer Linear Programming (ILP) based optimization to generate the shortest flight respecting the accuracy and point density constraints (\secref{s:slam-phase}). We call this the model collection flight.
% End before

% After
\item This paper presents a novel optimization formulation for obtaining 3D flight trajectories that capture 3D models of large buildings while maximizing SLAM positioning accuracy, minimizing flight duration, and capturing the given 3D model at a user-defined point density.
Point density, the number of points per unit area, allows the user to control the level-of-detail of the 3D model.
To achieve this, \sysname performs an exhaustive parameter search to find optimal flight parameters that minimize positioning error, determines the effective region of the LiDAR point cloud that satisfies the point density constraint, and uses an Integer Linear Programming (ILP) based optimization to generate the shortest flight respecting the accuracy and point density constraints (\secref{s:slam-phase}). We call this the model collection flight.

\item Even with careful designed trajectories, SLAM can accumulate drift error.
To counter this, \sysname continuously detects excessive SLAM drift with a novel algorithm that tracks SLAM and GPS position estimates.
% SLAM trajectory against GPS positions.
% This algorithm is robust to GPS error. 
When position estimates diverge significantly, signalling drift error, \sysname re-directs the drone to a designated origin (\secref{s:drift-est}); this effects a loop closure in SLAM and starts a new session, both minimize error~\cite{slam_part1,slam_part2}.

\item To optimize drone battery usage, before the model collection flight, \sysname uses a cheap reconnaissance flight along with a robust and efficient geometry extraction algorithm to locate buildings in the area of interest (\secref{sec:recon}).
This way, \sysname can focus model collection flights on the building and preserve the drone's battery.
% before conducting model collection flights. This approach minimizes the need to exhaust battery resources during the model collection process (\secref{sec:recon}).


% \item \sysname’s careful model collection can exhaust a drone’s battery. If a building’s location and shape are not known apriori, it is more efficient to expend some battery \sout{resources} \addraj{resource} to find the building in an area of interest, so \addraj{the} model collection flights can focus on the area where the building is located. To this end, \sysname introduces a robust and efficient geometry extraction algorithm using a cheap reconnaissance flight before model collection (\secref{sec:recon}).

\item \sysname offloads computation to a cloud server by compressing point clouds on the drone to the point where they can be transmitted over LTE (\secref{s:compression}). It processes these point clouds at LiDAR frame rate and with minimal end-to-end processing delay. 

\end{itemize}

{\small
\begin{table}
  \centering
  % \footnotesize
  \begin{tabular}{c c} \hline \hline
    \textbf{Challenge} & \textbf{Mechanism} \\ \hline 
    % \hline
    Model accuracy & Model collection trajectory planning \\ 
    Drift accumulation & Flight re-calibration\\ 
    Limited battery & Cheap reconnaissance flight\\ 
    Limited compute & Offloading compressed point clouds\\ \hline
  \end{tabular}
  \caption{Challenges and contributions}
  % \raj{Since we say trajectory planning, should we call "Compressed point cloud offloading"}}
  \label{tab:challenges}
\end{table}
}

Experiments (\secref{sec:eval}) with a complete \sysname implementation on real-world flights and a photorealistic drone simulator (AirSim~\cite{airsim}) demonstrate that \sysname can reconstruct 3D models on-the-fly (in hundreds of milliseconds after flight completion), within 10~cm accuracy, even after compressing 3D point clouds up to two orders of magnitude, and streaming them over LTE, for a variety of building shapes and sizes.
This makes \sysname \textit{faster}, and \textit{more accurate} than existing state-of-the-art photogrammetry~\cite{colmap}, and LiDAR-based 3D reconstruction~\cite{zhang2014loam, Cartographer} approaches. To our knowledge, \sysname is the first to demonstrate on-line, cloud-based, autonomous, accurate, 3D model reconstruction\footnote{The focus of this paper is on outdoor 3D reconstruction. Indoor reconstruction with smartphones or mobile devices is an orthogonal problem because their sensors have low range, and resolution. We have left an examination of this to future work.}.

% Points to make
% sysname can build 3D models in under a second, within 10cm accuracy, after compressing 3D point clouds upto two orders of magnitude, for a variety of building shapes and size.
% this makes it faster, and more accurate making it both faster and more accurate than both state-of-the-art photogrammetry and LiDAR-based approaches

% Experiments (\secref{sec:eval}) on real-world drone flights and a photo-realistic drone simulator (AirSim~\cite{airsim}) demonstrate that \sysname can achieve under 10~cm reconstruction accuracy for a wide range of building shapes and sizes, even after compressing the raw sensor data by almost two orders of magnitude. \sysname is \textit{faster} than  a state-of-the-art photogrammetry based approach~\cite{colmap}.
% % and LiDAR-based approaches~\cite{loam, cartographer}.
% % It is approach~\cite{colmap}, 
% It is also \textit{more accurate} than both photogrammetry and LiDAR-based approaches~\cite{zhang2014loam, Cartographer} because they cannot re-calibrate mid-flight. 

% % An experiment using the 
% A complete \sysname implementation on a drone
% is able to stream compressed point clouds over LTE, 
% can reconstruct the 3D model on-the-fly and deliver an accurate 3D model under a second after flight completion. To our knowledge, \sysname is the first to demonstrate on-line, cloud-based, autonomous, accurate, 3D model reconstruction\footnote{The focus of this paper is on outdoor 3D reconstruction. Indoor reconstruction with smartphones or mobile devices is an orthogonal problem because their sensors have low range, and resolution. We have left an examination of this to future work.}.
% \raj{Should we say "under a second" or "in hundreds of milliseconds"? "Under a second" is too conservative, since we are doing much better.}

% \wordcount

% \parab{Optimization formulation.}
% \sysname's main contribution is a novel optimization formulation to generate minimum flight length 3D trajectories that capture the physical structure at maximum accuracy. 
% Like photogrammetry, SLAM's tracking accuracy depends on trajectory design.
% Because of the drone's aerial view-point, point clouds captured from the drone are very sparse \ie they only contain returns from 9\% of all lasers fired from the LiDAR.
% Sparser point clouds make it difficult for SLAM to track the drone's motion.

% Moreover, with the drone's limited battery life,  
% Unlike autonomous vehicles, from an aerial drone's view-point, a LiDAR only receives 9\% of laser pulses return 3D coordinates.
% T
% Like photogrammetry, SLAM is sensitive to trajectory design.
% Like photogrammetry, SLAM is also sensitive to trajectory design.

% offloads SLAM to the cloud is computationally in
% To build a 3D model, \sysname must accurately track the drone's motion and align 3D point clouds.
% \sysname uses a LiDAR-mounted drone and a cloud-service to build high-fidelity 3D models.
% % The drone is equipped with a LiDAR, a cellular radio, and a compute source.
% % LiDAR-mounted drone and a cloud service to build high-fidelity 3D models of large physical structures. 
% Unlike cameras, \sysname actively perceives depth with a LiDAR that generates 3D point clouds.
% As it does, the drone instantly streams perceived point clouds to a cloud service.
% Then, the cloud service instantly positions each point cloud in a single coordinate system to build a 3D model.
% In doing so, it continuously monitors the quality of the 3D model and adjusts the trajectory of the drone in-flight for better 3D reconstruction.

% Hello world

% To position 3D point clouds, \sysname uses a LiDAR SLAM algorithm~\cite{Cartographer} because GPS can be inaccurate.
% However, the viewpoint from a drone is challenging for out-of-the-box SLAM algorithms and hence they lose track of the drone's motion.
% So, the trajectory design for SLAM-based 3D reconstruction is critical and determines the 3D model quality.
% Moreover, drones have limited battery life.
% These two competing constraints make  
%  SLAM cannot track the drone's motion because the view-point from a drone
 
% \sysname's primary contribution is an optimization formulation to obtain minimal duration 3D flight trajectories whilst ensuring high-quality 3D reconstruction.
%   first contribution 
% Trajectory optimizatoin
% The cloud service accurately positions the received point clouds with LiDAR SLAM to build the 3D model.


% which enables fast, and accurate 3D reconstruction from drones.
% entire process can take several days to can result in a turnaround time of several days.
% If the trajectory is not carefully crafted, the reconstructed 3D model might contain missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive. On a relatively powerful GPU workstation, reconstructing a building takes upto 8~hours (\secref{sec:eval}). As such, multiple iterations can result in a turnaround time of several days.

% What is the state of the art and what is wrong with the state-of-the-art
% \parab{State-of-the-art 3D reconstruction.}
% Most existing work (\secref{sec:related}) uses \textit{photogrammetry} to \textit{infer} 3D models from a sequence of 2D images captured either using drone-mounted cameras~\cite{7139681, 7989530, 8124461, 8628990} or by humans using ordinary mobile devices~\cite{company_hover}. 
% % Photogrammetry \textit{infers} 3D models using a technique known as multi-view stereo~\cite{furukawa15:_multi_view_stereo}, 
% Photogrammetry combines information from successive images, together with information about local motion, and inferred camera parameters such as the focal length. 
% Because photogrammetry approaches estimate depth from 2D images, their reconstruction times are relatively large \ie from several hours to days~\cite{company_drone_deploy} for large structures.
% Moreover, 


% \parab{Towards real-time 3D reconstruction.} 
% The nascent drone-based reconstruction industry is starting to use the \textit{time-to-reconstruction} as an important market discriminator. Startups promise to deliver models in hours or within a day~\cite{company_drone_deploy} after drone data collection. This trend has inspired newer, more time-sensitive applications of 3D modeling like (a) post-disaster reconstruction for search and rescue missions~\cite{drone_disaster_relief_1, drone_disaster_relief_2, drone_disaster_relief_3, drone_disaster_relief_4, drone_disaster_relief_5}, (b) construction site monitoring~\cite{company_drone_deploy}, (c) mapping mines, cell-towers and tunnels~\cite{hovermap, Prometheus}, (d) documenting interior office spaces~\cite{company_kaarta}, and (e) perhaps, most compelling, between-flight modeling of aircraft fuselages or blimps to determine structural integrity~\cite{company_austrian_airline}.

% Though startups are starting to promise smaller reconstruction times~\cite{hovermap,Prometheus}, they reconstruct 3D models \textit{offline} \ie after the drone has landed. Only one company we know of so far promises \textit{real-time} reconstruction~\cite{company_kaarta}, employing a human-operator holding a hand-held kit with a stereo camera (instead of a drone) to reconstruct interior spaces. 

% \parab{The Goal. } Given this, we want to \textit{accurately} reconstruct large 3D structures in \textit{near real-time}, with \textit{no human-intervention}.

% What were the applications of those 3D models in the past?
% \parab{Photogrammetry based reconstruction.}
% Most existing work (\secref{sec:related}) uses \textit{photogrammetry}, which takes as input a sequence of 2D camera images (and the positions associated with these images), captured either using drone-mounted cameras~\cite{7139681, 7989530, 8124461, 8628990} or by humans using ordinary mobile devices~\cite{company_hover}. Photogrammetry \textit{infers} 3D models using a technique known as multi-view stereo~\cite{furukawa15:_multi_view_stereo}, which combines information from successive images, together with information about local motion, and inferred camera parameters such as the focal length. Photogrammetry approaches estimate depth from 2D images so their reconstruction times are relatively large \ie from several hours to days~\cite{company_drone_deploy} for large structures.

% \parab{LiDAR-based reconstruction.}
% Unlike photogrammetry, LiDAR-based reconstruction can more directly infer 3-D models, because LiDARs directly provide depth information (unlike cameras). A LiDAR sensor measures distances to surfaces using lasers mounted on a mechanical rotating platform. The lasers and mechanical rotator sit within the enclosure of the LiDAR sensor. With each revolution of the lasers, the sensor returns a point cloud, or a \textit{LiDAR frame}. The point cloud is a set of 3D data points, each corresponding to a distance measurement of a particular position of the surrounding environment from the LiDAR. For instance, an Ouster OS1-64 LiDAR has 64 lasers that scan at 20~Hz, with a horizontal and vertical field of view of 360$\degree$ and 45$\degree$ respectively.

% To reconstruct a structure \eg a building, it suffices, in theory, to \textit{merge} points clouds captured from different locations around the building. To understand what it means to merge point clouds, consider two successive clouds $p$ and $p'$. A point $x$ on the surface of the building may appear both in $p$ and $p'$. However, since the drone has moved, this point $x$ appears at different positions (relative to the LiDAR) in the two point clouds. If we precisely transform both point clouds to the same coordinate frame of reference, then the union of points in $p$ and $p'$ constitutes part of the 3D model of the building. 

% \parab{Accurate positioning ensures high-quality models.}
% This requires the precise position of the LiDAR at the positions where it captured the point clouds. The accuracy of positioning determines model quality. Two metrics define quality. \textit{Accuracy}, the average distance between the position of a point in the model and the corresponding point on the surface (see \secref{sec:design} for a more precise definition), clearly relies on accurate positioning. \textit{Completeness}, the degree to which a model captures the entire structure, also relies on accurate positioning, since positioning errors can lead to gaps in the captured model.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\columnwidth]{figs/fig_slam_vs_gps_3d_model.pdf}
%     \caption{GPS-derived (left), SLAM-derived (middle), and \sysname-derived (right) models of a large complex on our campus.
%     \label{fig:slam_vs_gps_3d_model}}
% \end{figure}

% \parab{Strawman: Using GPS for positioning.}
% Because drones can carry GPS receivers, GPS can be used to position point clouds. Unfortunately, GPS errors can be several meters in obstructed settings, resulting in poor accuracy and completeness of the 3D model. The left image of \figref{fig:slam_vs_gps_3d_model} shows a 3D model of a building assembled using a drone flight over a commercial building; the building's outline is fuzzy, as are the contours of the trees surrounding the building. The right image shows a 3D reconstruction using techniques proposed in this paper, which does not use GPS. (All reconstructions in \figref{fig:slam_vs_gps_3d_model} use real data captured from a drone-mounted LiDAR~\secref{sec:eval}).

% High-precision GNSS/RTK receivers can provide more accurate positioning but require additional infrastructure, are costly, and can perform poorly in urban environments due to non line-of-sight signals that degrade accuracy (\eg prior work~\cite{Carloc} reports that RTK-enabled receivers can exhibit tens of meters error in downtown environments). Prior work~\cite{uav_lidar_1,uav_lidar_2} has used expensive GPS receivers in the context of \textit{remote sensing}, using specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors (but for \textit{offline} model reconstruction). In contrast, in this paper we consider solutions that employ off-the-shelf technologies: drones, and commodity GPS and LiDAR.

% \parab{An alternative: Using SLAM for positioning.}
% LiDAR SLAM (Simultaneous Localization And Mapping~\cite{slam_part1, slam_part2}) algorithms can provide accurate \textit{pose} (position and orientation) estimates, which can be used to position point clouds. These algorithms use scan or feature matching techniques to align consecutive LiDAR frames to determine the pose of the drone throughout its flight. For example, scan matching uses techniques~\cite{icp} to find the closest match for each point in the source point cloud $\mathbf{A}$ to a point in the reference point cloud $\mathbf{B}$. It then estimates the transformation (translation and rotation) that best aligns each point in $\mathbf{A}$ to its corresponding point in $\mathbf{B}$. By repeating this process across consecutive LiDAR frames, SLAM can position each frame in the first frame's coordinate frame of reference.



==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}
% Set up/motivate the problem carefully:
% - Define accuracy and completeness

% - Can use LiDAR, and LiDAR SLAM
%   - Show what happens when we do
%   - SLAM loses tracking
% - Challenge:
%   - Figure out how to minimize tracking loss by trajectory generation
%   - May still have drift; online re-calibrate

% Define Accuracy and Completeness

In this section, we provide results from experiments that motivate \sysname's approach. 
% Before we do this, we describe metrics that capture the quality of 3D reconstruction.

% \parab{Quantifying 3D model quality. }
% Prior work on 3D reconstruction~\cite{reconstructionmetrics} has proposed two metrics, \textit{accuracy} and \textit{completeness}.
% Consider a 3D model $M$ and a corresponding ground-truth $M_g$. 
% Accuracy describes how \textit{closely} the 3D model $M$ resembles the ground truth $M_g$. 
% Accuracy is the root mean-square error (RMSE) of the distance from each point in $M$ to the nearest point in $M_g$. 
% Completeness describes \textit{what extent} of the ground truth $M_g$ the 3D model $M$ captures.
% Completeness is the RMSE of the distance from each point in $M_g$ to the nearest point in $M$. 

% To put these numbers in context, a 10~cm accuracy means that every point on 3D model $M$ is displaced by 10~cm, on average, from its ground truth position in $M_g$.
% % A high accuracy value means the 3D model $M$ does not resemble the ground truth $M_g$.
% A 50~cm completeness means that, on average, for every point on the ground truth $M_g$, the nearest point on the 3D model $M$ is 50~cm away.
% % A high completeness value means the 3D model $M$ is an incomplete representation of the ground truth $M_g$.
% If both accuracy and completeness are zero, $M$ perfectly matches $M_g$.
% So, for both metrics, \textit{lower is better}. 
% If $M$ captures all points in $M_g$, but the positions of the points are erroneous, then both accuracy and completeness will be non-zero. 
% If $M$ captures only one point in $M_g$, but positions it correctly, its accuracy is perfect, but completeness is poor. 
% These two metrics are roughly analogous to precision (accuracy) and recall (completeness).
% \fawad{Consider adding a figure to show how these metrics work. Maybe with MVS}

% \begin{figure}[t]
%  \centering
%  \begin{subfigure}{0.49\linewidth}
%  \includegraphics{figs/fig_incomplete_mvs.pdf}
%  \caption{MVS reconstruction (right image) of a large building (left image shows ground truth 3D model).}
%  \label{fig:mvs}
% \end{subfigure}
% \begin{subfigure}{0.49\linewidth}
%     \centering
%     \includegraphics{figs/fig_slam_vs_gps_3d_model.pdf}
%     \caption{GPS (left), SLAM (middle), and \sysname (right) derived models of a large complex on our campus. All models are color-coded with the same height ramp function.}
%     \label{fig:slam_vs_gps_3d_model}
% \end{subfigure}
% \caption{3D reconstructions using MVS, SLAM, and GPS.}
% \end{figure}


% \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.7\columnwidth]{figs/fig_slam_challenge.pdf}
%  \caption{LiDAR returns when mounted on a vehicle and a drone platform}
%  \label{fig:slam_challenge}
% \end{figure}

\begin{figure}[t]
 \centering
  \includegraphics[width=0.5\columnwidth]{figs/fig_incomplete_mvs.pdf}
 \caption{\add{An MVS/photogrammetry-based 3D reconstruction of a building (right image) can contain missing regions. The left image shows the ground truth 3D model.}}
 \label{fig:mvs}
\end{figure}

{\small
\begin{table}
  \centering
  % \footnotesize
  % \begin{subtable}{0.45\linewidth}
  \begin{tabular}{{c  c  c  c}} \hline \hline
    \textbf{Building} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} & \textbf{Time (s)} \\ \hline
    % \hline
    Small  & 0.11 & 0.80 & 23084 \\ 
    Large  & 0.16 & 0.75 & 31600 \\ \hline
  \end{tabular}
  \caption{\add{Photogrammetry can be slow, inaccurate and incomplete. The small building is 50~m~x~50~m~x~20~m, the large is 100~m~x~50~m~x~20~m.}}
  \label{tab:mvs_motiv}
\end{table}
}




\parab{Drone-based photogrammetry can be slow and inaccurate.} 
% Photogrammetry \textit{infers} 3D models using multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS). MVS algorithms infer the structure (position, and orientation) of the scene from the set of images. Using this structure and stereo correspondence from multiple images, these algorithms estimate the depth of every pixel in each image. A fusion of these 3D points generates a dense 3D reconstruction of the entire scene/object. Though MVS 3D reconstructions are generally accurate, they may contain missing regions or holes~\cite{furukawa15:_multi_view_stereo} which arise if MVS cannot confidently estimate their depths from the set of images.
Today, to build a 3D model, a drone operator flies a drone in a given trajectory to collect 2D images. Then, the operator uploads these images to a cloud service after the drone lands. The cloud service runs an MVS algorithm to build a 3D model. If the model contains missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive.

To quantify these shortcomings, we conducted an experiment (methodology described in~\secref{sec:eval}) in which we used the most widely used open source implementation of MVS (ColMap~\cite{colmap}) to reconstruct a 3D model of two buildings. For each building, we tried several trajectories, and selected the one that provided the highest quality model. \tabref{tab:mvs_motiv} shows these values, and \figref{fig:mvs} is a visual illustration for that highest quality flight. 
% \figref{fig:mvs} is a visual illustration of highest quality flight MVS reconstruction. 
The left image shows the ground truth model whereas the right image shows the 3D model from the MVS reconstruction. Accuracy is slightly higher than 10~cm; this is desirable. Completeness, however, even for the best flight is 75~cm or more (right image in \figref{fig:mvs} illustrates many regions in the MVS reconstruction are incomplete); \sysname achieves 5 to 9~cm completeness (\secref{sec:eval}, almost an order of magnitude better). Finally, MVS requires nearly 7-9 \textit{hours} to reconstruct the model;  \sysname assembles the model in-flight, so the model is ready immediately after the drone lands.


In theory, photogrammetry could detect, in-flight, when the model might be incomplete and adapt the trajectory accordingly. This has proven to be hard to do without running the entire MVS pipeline~\cite{mostegel2016uav, 7422384} on the set of images. To minimize iterations, practitioners have developed rules of thumb for designing trajectories (such as taking highly-overlapping uniformly-illuminated images of texture-rich surfaces)~\cite{colmap, dd_guidelines}, but realize there is no way to ensure complete and high-quality 3D reconstruction without iteration~\cite{mostegel2016uav}. So, companies hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} who have developed trajectory design intuitions over time.

% \textit{\textbf{Takeaway: }Photogrammetry reconstruction can be inaccurate and its quality depends on the drone's flight trajectory. Because photogrammetry is also slow,  there is no way to  depends on the trajectory used to collect 2D images, and slow and can be inaccurate


\parab{Other alternatives for positioning are unsuitable.}
Because drones can carry GPS receivers, GPS can be used to position point clouds. Unfortunately, GPS errors can range up-to several meters~\cite{gnome}, resulting in poor accuracy and completeness of the 3D model. The left image of \figref{fig:slam_vs_gps_3d_model} shows a 3D model of a building assembled using a drone flight over a commercial building that uses GPS for positioning; the building's outline is fuzzy, as are the contours of the trees surrounding the building. \tabref{tab:slam_gps_reconstruction} shows that the accuracy and completeness for the GPS reconstructed model are 1.6~m and 0.53~m respectively, both of which are undesirable. The right image shows a 3D reconstruction using techniques proposed in this paper, which does not use GPS. (All reconstructions in \figref{fig:slam_vs_gps_3d_model} use real data captured from a drone-mounted LiDAR~\secref{sec:eval}).




% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=\columnwidth]{figs/fig_slam_vs_gps_3d_model.pdf}
% %     \caption{GPS (left), SLAM (middle), and \sysname (right) derived models of a large complex on our campus. All models are color-coded with the same height ramp function.}
% %     \label{fig:slam_vs_gps_3d_model}
% % \end{figure}

% \begin{table}[t]
%   \centering
%   \footnotesize
%   \begin{tabular}{{|c|c|c|}} \hline
%     \textbf{Approach} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} \\ \hline
%     % \hline
%     GPS  & 1.60 & 0.53 \\ \hline
%     SLAM  & 2.30 & 1.30 \\ \hline
%     \sysname & 0.13 & 0.09 \\ \hline
%   \end{tabular}
%   \caption{Relative to \sysname, alternative reconstruction approaches for drone-based LiDAR reconstruction give poor quality 3D models.}
%   \label{tab:slam_gps_reconstruction}
% \end{table}

% \begin{figure}[t]
%  \centering
%  \begin{minipage}{0.37\linewidth}
%  \includegraphics{figs/fig_incomplete_mvs.pdf}
%  \caption{MVS reconstruction (right image) of a large building (left image shows ground truth 3D model).}
%  \label{fig:mvs}
% \end{minipage}
% \hfill
% \begin{minipage}{0.59\linewidth}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/fig_slam_vs_gps_3d_model.pdf}
    \caption{\add{The figure shows three models of a large complex on our campus: GPS (left), SLAM (middle), and \sysname (right). All models use the same height ramp function to color-code the z-axis, with blue representing the lowest points and orange representing the highest. The \sysname model has distinct features and trees, with clear and crisp coloring, indicating a good reconstruction. In contrast, the GPS and SLAM models have diffused colors and lack visible features, suggesting poor and noisy reconstructions.}}
    \label{fig:slam_vs_gps_3d_model}
% \end{minipage}
% \caption{3D reconstructions using MVS, SLAM, GPS, and \sysname.}
\end{figure}

{\small
\begin{table}
  \begin{tabular}{{c c c c}} \hline \hline
    \textbf{Approach} & \textbf{Accuracy (m)} & \textbf{Completeness (m)} & \add{\textbf{Flight time (s)}} \\ \hline
    % \hline
    GPS  & 1.60 & 0.53 & - \\ 
    SLAM  & 2.30 & 1.30 & - \\ 
    \sysname & 0.13 & 0.09 & - \\ \hline
  \end{tabular}
  \caption{Relative to \sysname, alternative reconstruction approaches for drone-based LiDAR reconstruction give poor quality 3D models.}
  \label{tab:slam_gps_reconstruction}
\end{table}
}
% \ramesh{Do we have acc/compl for GPS?}
% \fawad{Yes, but we have it for the real-world building not the Airsim ones. I added the numbers in the paragraph above.}

High-precision GNSS/RTK receivers can provide more accurate positioning but require additional infrastructure, are costly, and can perform poorly (tens of meters error~\cite{Carloc}) in urban environments due to non line-of-sight signals that degrade accuracy. Prior work~\cite{uav_lidar_1,uav_lidar_2} has used expensive GPS receivers in the context of \textit{remote sensing}, using specialized unmanned aerial vehicles (UAVs) with long-range LiDAR sensors (but for \textit{offline} model reconstruction). In contrast, in this paper we consider solutions that employ off-the-shelf technologies: drones, and commodity GPS and LiDAR for online reconstruction.

\parab{SLAM-based positioning on a drone is challenging.}
LiDAR-based SLAM algorithms continuously align 3D point clouds using scan~\cite{Cartographer}, and feature matching~\cite{zhang2014loam,liosam} techniques to precisely estimate the pose (position, and orientation) of the LiDAR/drone. The accuracy of position estimates is dependent on SLAM's ability to precisely align 3D point clouds. Alignment, in turn, depends on the nature of the 3D point clouds. For instance, it is relatively easier to align two 3D point clouds for a slow-flying drone because consecutive point clouds are captured in close proximity. 

Although SLAM is used in autonomous driving (among other applications) for precise positioning, it is challenging to use it out-of-the-box on a drone. 
When mounted on a drone, a LiDAR generates significantly sparser 3D point clouds as compared to a vehicle.
Sparsity makes it difficult for the SLAM algorithm to align the point clouds, resulting in imprecise positioning.

% To explain this, consider \figref{fig:slam_challenge} which 
On a vehicle, as shown in \figref{fig:slam_challenge} (A), the LiDAR is placed such its scan plane is parallel to the ground.
What this means is: the central laser beams originating from of the LiDAR (such as those striking with the stop sign) run parallel to the ground.
In this orientation, the vehicle-mounted LiDAR receives returns from numerous objects (shown by the straight orange lines) \eg the road, traffic signs, buildings, other vehicles \etc
% because the vehicle has objects closeby, the LiDAR generates a lot of returns.
On a drone hovering at height $h$ with a LiDAR in the same orientation, it will have very few returns (if any) as depicted in \figref{fig:slam_challenge} (B).
% It will only get returns from objects below the drone
This is because, while in-flight, the only returns for the drone will be from the buildings/ground below it.

% because the drone is in-flight and ground/buildings are below the drone.
A different way to orient the LiDAR is to position it such that the scan plane of the LiDAR is perpendicular to the ground (\figref{fig:slam_challenge} (C)) .
In this orientation, the LiDAR receives relatively more returns as compared to \figref{fig:slam_challenge} (B).
Even then, these returns are a small fraction (only 1/10th) of the returns from a vehicle mounted LiDAR.
% In the vehicle case, \figref{fig:slam_challenge} (A), the LiDAR receives returns from 360\degree on the horizontal axis whereas for the drone case, \figref{fig:slam_challenge} (C), the LiDAR only receives returns from 45\degree that hit the ground surface.
With sparse returns, SLAM cannot precisely align consecutive point clouds and hence results in imprecise and inaccurate positioning.
As such, we find that positioning accuracy in SLAM is critically dependent on the drone's \textit{flight trajectory}.

% Consider an 8-beam LiDAR as shown in \figref{fig:fig_slam_challenge}.
% These laser beams are radially placed on a rotating platform in a mechanical closure.
% Each laser beam shoots laser pulses in 360\degree.
% Because the lasers are radially placed, the beams diverge as their distance from the LiDAR increases.
% These laser beams are radially placed in the mechanical enclosure of the LiDAR.
% Thereby, the LiDAR receives more returns from the same object when placed closeby as opposed to when it placed far away.
% Objects closeby to the LiDAR generate more returns because the LiDAR beams have not yet dispersed.
% Objects that are far away generate fewer returns because LiDAR beams have dispersed.

\begin{figure}[t]
\centering
\begin{minipage}{0.65\linewidth}
 \includegraphics{figs/fig_slam_challenge.pdf}
 \caption{LiDAR returns when mounted on a vehicle (A) and a drone platform (B and C). The solid lines indicate the lasers have hit an object whereas the dotted lines that those laser beams did not hit any object.}
 \label{fig:slam_challenge}
\end{minipage}
\hfill
\begin{minipage}{0.3\linewidth}
 \includegraphics{figs/rectflight.png}
 \caption{Rectilinear trajectory for SLAM-based reconstruction.}
 \label{fig:rectflight}
\end{minipage}
% \caption{}
\end{figure}

\figref{fig:slam_vs_gps_3d_model} (middle) shows reconstruction using SLAM from a rectilinear flight (\figref{fig:rectflight}) that ensures building coverage. For this flight, the accuracy and completeness are 2.3~m and 1.3~m respectively (\tabref{tab:slam_gps_reconstruction}, lower values of accuracy and completeness are better), orders to magnitude higher than \sysname-based reconstruction. This reconstruction is visually worse than \sysname-based reconstruction (\figref{fig:slam_vs_gps_3d_model} (right)), because the underlying SLAM algorithm is unable to \textit{track} LiDAR frames (\ie it is unable to match points in successive point clouds). \sysname, which layers trajectory generation and drift re-calibration on top of SLAM is significantly more accurate and complete. For SLAM-based reconstructions, we used the Google Cartographer~\cite{Cartographer} LiDAR SLAM implementation which uses scan matching.


% As such, positioning accuracy in SLAM critically depends on the drone's \textit{flight trajectory}.

% \figref{fig:slam_challenges} illustrates the positioning of a LiDAR on a vehicle and a drone. On a vehicle, as the 

% \parab{SLAM-based positioning can be inaccurate.}
% Even with SLAM, reconstruction quality is critically dependent on the design of the drone \textit{trajectory}. 
% \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.35\columnwidth]{figs/rectflight.png}
%  \caption{Rectilinear trajectory for SLAM-based reconstruction.}
%  \label{fig:rectflight}
% \end{figure}

% To quantify the quality of SLAM-based reconstruction, we measured accuracy and completeness for the two buildings discussed above. These experiments (and all others in this paper) use Google's Cartographer~\cite{Cartographer}, a recent implementation of LiDAR SLAM. As \tabref{tab:slam_motiv} shows, SLAM-based reconstruction has worse accuracy than MVS, but better completeness. \sysname, which layers trajectory generation and drift re-calibration on top of SLAM is significantly more accurate and complete (\secref{sec:eval}).

% \fawad{These numbers are very low (they need to be higher). They represent \sysname without re-calibration. For GPS and unoptimized SLAM, maybe we can just use numbers from the real-world trace instead?}
% \begin{table}[h]
%   \small
%   \centering
%   \begin{tabular}{{|l|c|c|c|}} \hline
%     Building & Accuracy (m) & Completeness (m)  \\ \hline\hline
%     Small  & 0.25 & 0.14 \\ \hline
%     Large  & 0.21 & 0.24 \\ \hline
%   \end{tabular}
%   \caption{SLAM-based reconstruction can be inaccurate. The dimensions of the buildings are as in \tabref{tab:mvs_motiv}.}
%   \label{tab:slam_motiv}
% \end{table}


% \noindent$\blacktriangleright$

\parab{Limited compute on drones.}
For \sysname to detect SLAM drift (\secref{sec:intro}) in-flight, it must run SLAM as the drone flies. However, existing SLAM algorithms \textit{cannot run at full frame rate} on mobile computing platforms mounted on drones. A DJI M600Pro (which we use in this paper) hexacopter has a maximum payload weight of 5~kg. It carries an A3Pro flight controller that contains three IMUs and three GNSS receivers. We have also mounted an LTE radio and an Ouster OS1-64 LiDAR, as well as a Jetson TX2 board. This compute capability is far from sufficient to run LiDAR SLAM\footnote{With a 64-beam LiDAR, SLAM processes upto 480 Mbps of 3D data}. 

On the TX2, we ran two popular, representative LiDAR-SLAM algorithms, Cartographer~\cite{Cartographer} and LOAM~\cite{zhang2014loam}.
In this experiment, both SLAM implementations use \sysname's optimized 3D flight trajectories. In \tabref{tab:lidar_slam_compute} we show accuracy, completeness and performance results for two the LiDAR SLAM algorithms. 
Cartographer, a scan matching algorithm, can only process 2 frames per second (LiDARs generate 10-20 frames per second) and LOAM, a feature-matching algorithm, can process 5 frames per second. Though faster, LOAM reconstructions are worse than Cartographer.

\begin{table}[t]
  % \footnotesize
  \centering
  \begin{tabular}{c  c  c} \hline \hline 
    \textbf{Metric} & \textbf{Cartographer~\cite{Cartographer}} & \textbf{LOAM~\cite{zhang2014loam}} \\ \hline
    % \hline
    Frame Rate (fps) & 2 & 5 \\ 
    Accuracy (m) & 0.21 & 5.75 \\ 
    Completeness (m) & 0.09 & 2.74 \\ \hline
  \end{tabular}
  \caption{LiDAR SLAM on Jetson TX2. For both accuracy and completeness, lower is better.}
  \label{tab:lidar_slam_compute}
\end{table}

We make two observations from \tabref{tab:lidar_slam_compute}.
First, Cartographer is a more accurate SLAM algorithm than LOAM for drone-mounted LIDAR. For this reason, \sysname uses Cartographer.
Second, neither SLAM implementation can run at full frame-rate on the drone. In particular, Cartographer runs only at 2~fps, but we need to process SLAM at full-frame rate to be able to detect drift in-flight, so \sysname offloads SLAM to the cloud.



These experimental results motivate the design of \sysname, which we now describe.


% Two metrics define the quality of a 3D model. 
% \textit{Accuracy} quantifies how closely a 3D model replicates a physical object (see \secref{s:slam-phase} for a more precise definition).
% It is the average Euclidean distance between the positions of every point in the 3D model to the corresponding point on the surface of the physical object (see \secref{s:slam-phase} for a more precise definition).
% A 3D model with an accuracy of 0~m perfectly replicates a physical object.
% \textit{Completeness} quantifies the degree to which a model captures the entire physical object (see \secref{s:slam-phase} for a more precise definition).
% It is the inverse of accuracy \ie it is the average Euclidean distance between the position of every point on the surface of the physical object to the corresponding point on the 3D model.
% A 3D model with 0~m completeness is completely perfectly a physical object.

% Photogrammetry
% - Show MVS doesn't work, and why
%   - Don't know which part is not captured well (do we have some examples)
% \parab{Multi-View Stereo (MVS). }
% % Photogrammetry uses multi-view stereo algorithms to infer a 3D model from drone captured 2D images.
% % MVS takes too long and there is no feedback signal into how the reconstruction is going.
% % Mostly using photogrammetry.
% Most existing work (\secref{sec:related}) use \textit{photogrammetry} to infer a 3D model from 2D images.
% Photogrammetry uses multi-view stereo~\cite{furukawa15:_multi_view_stereo}, which takes as input a sequence of 2D camera images (and the positions associated with these images), captured either using drone-mounted cameras~\cite{7139681, 7989530, 8124461, 8628990} or by humans using ordinary mobile devices~\cite{company_hover}. 
% % Photogrammetry \textit{infers} 3D models using multi-view stereo~\cite{furukawa15:_multi_view_stereo} (MVS). 
% MVS algorithms infer the structure (position, and orientation) of the scene from the set of images (called structure from motion or SfM). 
% Using this structure and stereo correspondence from multiple images, these algorithms estimate the depth of every pixel in each image. 
% A fusion of these 3D points generates a dense 3D reconstruction of the entire scene/object.

% \parab{No feedback signal in MVS. }
% Though MVS 3D reconstructions are generally accurate, they may contain missing regions or holes~\cite{furukawa15:_multi_view_stereo} which arise if MVS cannot confidently estimate their depths from the set of images.

% Collect good images or have an expert do it and hope for the best.
%Besides some generic rules of thumb for collecting images (\eg texture-rich, uniform illuminated images with high overlap taken from diverse viewpoints)~\cite{colmap, dd_guidelines}, there is no way to ensure complete and high-quality 3D reconstruction~\cite{mostegel2016uav}. Companies, besides issuing these guidelines,  hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} for data collection who have developed intuition over time for better trajectory design.

% It feels important to talk about this work but it might also raise questions about our contributions from the very start. I am not sure if we should keep it or remove it (it is already present in the related work section)
% There is work~\cite{cvpr} that trains a model to predict the likelihood of a good/complete 3D model from a set of images. However, this model is specific to a given dataset and a given MVS algorithm. For a different scene or MVS algorithm, the model will need to be trained again with a new set of labeled data.

% MVS takes too long and there is no feedback signal into how the reconstruction is going.
% Today, to build a 3D model, a drone operator flies a drone in a given trajectory to collect 2D images. Then, the operator uploads these images to a cloud service after the drone lands. The cloud service runs an MVS algorithm to build a 3D model. If the model contains missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive. On a relatively powerful GPU workstation, reconstructing a building takes upto 8~hours (\secref{sec:eval}). As such, multiple iterations can result in a turnaround time of several days.

% \parae{The need for trajectory adaptation.}
% In theory, photogrammetry can avoid this iterative approach if it could detect, in-flight, when the model might be incomplete and adapt the trajectory accordingly. This has proven to be hard to do without running the entire MVS pipeline~\cite{mostegel2016uav, 7422384} on the set of images. To minimize  iterations, practitioners have developed rules of thumb for designing trajectories (such as taking highly-overlapping uniformly-illuminated images of texture-rich surfaces from diverse viewpoints)~\cite{colmap, dd_guidelines}, but realize there is no way to ensure complete and high-quality 3D reconstruction without iteration~\cite{mostegel2016uav}. For this reason, companies hire drone pilots/photogrammetrists~\cite{mvslessons, photogrammetryissues} who have developed trajectory design intuitions over time.

% Today, to build a 3D model, a drone operator flies a drone in a given trajectory to collect 2D images. Then, the operator uploads these images to a cloud service after the drone lands. The cloud service runs an MVS (multi-view stereo) algorithm to build a 3D model. If the model contains missing regions (detected by visual inspection), the operator adjusts the trajectory and flies the drone again~\cite{mvslessons, photogrammetryissues}. It can take multiple iterations to get the desired 3D model. Moreover, MVS algorithms are compute-intensive. On a relatively powerful GPU workstation, reconstructing a building takes upto 8~hours (\secref{sec:eval}). As such, multiple iterations can result in a turnaround time of several days.



==> refs.tex <==
\bibliography{references.bib}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

